Classification of Edge-dependent Labels of Nodes in Hypergraphs

A hypergraph is a data structure composed of nodes and hyperedges, where each hyperedge is an any-sized subset of nodes. Due to the flexibility in hyperedge size, hypergraphs represent group interactions (e.g., co-authorship by more than two authors) more naturally and accurately than ordinary graphs. Interestingly, many real-world systems modeled as hypergraphs contain edge-dependent node labels, i.e., node labels that vary depending on hyperedges. For example, on co-authorship datasets, the same author (i.e., a node) can be the primary author in a paper (i.e., a hyperedge) but the corresponding author in another paper (i.e., another hyperedge). In this work, we introduce a classification of edge-dependent node labels as a new problem. This problem can be used as a benchmark task for hypergraph neural networks, which recently have attracted great attention, and also the usefulness of edge-dependent node labels has been verified in various applications. To tackle this problem, we propose WHATsNet, a novel hypergraph neural network that represents the same node differently depending on the hyperedges it participates in by reflecting its varying importance in the hyperedges. To this end, WHATsNet models the relations between nodes within each hyperedge, using their relative centrality as positional encodings. In our experiments, we demonstrate that WHATsNet significantly and consistently outperforms ten competitors on six real-world hypergraphs, and we also show successful applications of WHATsNet to (a) ranking aggregation, (b) node clustering, and (c) product return prediction.

==> backup/000abstract.tex <==
Hypergraphs represent group interactions (e.g., collaborations of researchers and discussions on online Q\&A platforms) more naturally and accurately than ordinary graphs. Since hypergraph modeling has been shown beneficial, a large number of hypergraph neural networks have been proposed.
However, most of them have been evaluated on node classification tasks where unique properties of hypergraph-structured data are overlooked. For example, on co-authorship datasets, %few authors do only the first author in their lifetime. Instead, 
the same author can be the primary author in a paper but the corresponding author in another paper. 

In this work, we introduce classification of edge-dependent node labels (i.e., node labels that vary depending on hyperedges), as a new problem, together with six real-world datasets. This problem can work as a new benchmark task for hypergraph neural networks, and its usefulness is verified in various applications, including ranking aggregation, node clustering, and product return prediction.

To tackle this problem, we also propose a novel hypergraph neural network, \method. 
% In order to make the influence of nodes different depending on which nodes are formed together one hyperedge, \method consists of attention modules \WithinAttention, which is designed to use interactions between nodes within the hyperedge, and positional encodings \PE. 
In order to make the influence of nodes different depending on hyperedges, \method represents a single node differently according to each hyperedge it involves. 
To this end, we propose the \WithinAttention module, which effectively models interactions among nodes within each hyperedge, with the help of the explicit relative information named \PE.
Through experiments, we demonstrate that \method is (a) \textbf{Accurate}:  showing the highest performance among nine competitors in six real-world hypergraphs, (b) \textbf{Complete}: the power of each component being proved by ablation studies, and (c) \textbf{Practical}:  achieving performance improvement in three  applications.

%% In a nutshell, \method represents a single node differently according to each hyperedge it involves. 
%% To this end, we propose a \WithinAttention, which effectively models interaction among nodes within each hyperedge, with the help of the explicit relative information named \PE.


==> backup/010intro.tex <==

% ---------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{figure}[t]
    % \vspace{-2mm}
    \begin{minipage}{0.63\linewidth}
        \includegraphics[width=1.0\textwidth]{FIG/mainfigure/ex1_2.jpg}
    \end{minipage}
    \begin{minipage}{0.34\linewidth}
        \vspace{0.2\linewidth}
        \includegraphics[width=1.0\textwidth]{FIG/mainfigure/ex2_3.jpg}
    \end{minipage}
    
    \begin{minipage}{1.3\linewidth} \small
         \hspace{0.02\linewidth} (a) Example data: Coauthors in publications \hspace{0.06\linewidth} (b) Hypergraph
    \end{minipage}
    %\hspace{0.05\linewidth}
    
    \caption{\label{fig:intro_ex} The three publications by the six authors in (a) are modeled as the hypergraph with six nodes and three hyperedges in (b). The labels of nodes indicate the orders of the authors (\underline{F}irst, \underline{L}ast, or \underline{O}thers) in each publication, and thus they are dependent on hyperedges.}
\end{figure}

% New StoryLine



% 1) Hypergraph
Real-world relationships are complex and often go beyond pairwise relations. For example, researchers co-author a paper with more than one other researcher, and people send emails to many receivers at once. A \textit{hypergraph} is a natural representation of these group relations. It consists of nodes and hyperedges, and each hyperedge is a subset of any number of nodes (see Figure~\ref{fig:intro_ex}).
Hypergraph modeling has shown advantages over ordinary graph modeling in node clustering~\cite{wolf2016advantages}, interaction prediction~\cite{yoon2020much}, and anomaly detection \cite{lee2022hashnwalk}, and it has been used in a variety of fields, including recommendation systems~\cite{xia2021self,hada2021hypertenet,qiu2021exploiting,ding2021hypergraph} and natural sciences~\cite{gu2020quantum}. 



% 2) Hypergraph Neural Network
% By following up the success of graph neural networks, 
In order to exploit the advantages of hypergraph modeling,
a large number of hypergraph neural networks have been proposed,
and they are typically evaluated on node classification tasks, whose objective is to predict global properties of nodes.
HGNN~\cite{feng2019hypergraph}, HCHA~\cite{bai2021hypergraph}, and HyperGCN~\cite{yadati2019hypergcn} transform hypergraphs into graphs to apply graph convolution. % to hypergraphs via clique-expansion, i.e., replacing hyperedges with cliques to obtain a graph.
% trains a graph convolutional network by replacing hyperedges with incomplete subgraphs.
HNHN~\cite{dong2020hnhn} alternately updates hypergraph embeddings and node embeddings via graph convolution. %  with an activation function on both steps.
%which makes differents from message passing in the clique-expansion graph. 
UniGNN~\cite{huang2021unignn} is a framework for generalizing classic graph neural networks (e.g., \cite{kipf2016semi,velivckovic2018graph}) directly to hypergraphs. % with the least effort
AllSet~\cite{chien2021you} is an expressive framework that includes all these hypergraph neural networks as special cases.

% 3) Hyperedge-dependent Node Role
%\red{KJ: Please add a figure for explaining hypergraphs and edge-dependent labels}

% In hypergraphs, the labels of nodes can vary depending on the hyperedges. For example, the author could be either a leading or a corresponding author in the publication. A sender of one email also can be a receiver of another email. In the Q\&A platforms, the same person can ask or answer in the post. However, most hypergraph neural networks have been evaluated on a typical node classification problem where one node is assigned one label. 


However, in many real-world hypergraphs, the property or role of each node varies depending on hyperedges that it is included in. For example, in co-authorship datasets, the same researcher can be the primary author in one paper but the corresponding author in another paper (see Figure~\ref{fig:intro_ex}). In email datasets, the same person can be a receiver of an email but CC'ed in another email. In online Q\&A platforms, the same person can be the questioner in a post but an answer in another post. These edge-dependent properties of nodes have been shown useful in various hypergraph-based tasks, including ranking aggregation~\cite{chitra2019random}, node clustering~\cite{hayashi2020hypergraph},  product-return prediction~\cite{li2018tail} and anomaly detection~\cite{lee2022hashnwalk}.


% In such cases, defining (and predicting) global node labels results in neglecting the rich edge-dependent characteristics of nodes,
% However, typical node classification tasks aims to understand the global characteristic of each node in a graph. 


% 4) Our contribution 1. Hypergraph Learning Benchmark & applications for ranking, anomaly detection
% In this work, we introduce a new classification task of edge-dependent labels of nodes as a benchmark for hypergraph neural network learning. 
% The goal is to correctly predict the unknown node labels of nodes which would be different according to what hyperedge it includes.
% The usefulness of considering nodes differently depending on hyperedges has already been proven, e.g. ranking applications~\cite{chitra2019random}, node clustering~\cite{hayashi2020hypergraph}, product return prediction~\cite{li2018tail} and anomaly detection~\cite{lee2022hashnwalk}.
% Furthermore, since edge-dependent node labels cannot be represented in the clique expansion graph, it is expected that our proposed classification task requires the utilization of higher relationships in the hypergraph.
% Lastly, this classification task would alleviate the limitation of the datasets for hypergraphs and help improve the expressive power and efficiency of hypergraph neural networks as a new benchmark.
In this work, we introduce classification of edge-dependent node labels in a hypergraph, as a new problem, together with six real-world datasets. The problem works as an effective hypergraph-learning benchmark task that is complementary to common benchmark tasks (e.g., node classification, hyperedge prediction and clustering) for three reasons.
First, it is proper to evaluate how well unique characteristics of hypergraphs are captured. 
Note that edge-dependent node labels are unique in hypergraphs, and especially they disappear in clique-expanded graphs, which are the result of direct simplification of hypergraphs into ordinary graphs.
Second, as shown in the experiment section, the problem cannot be solved satisfactorily by global node and hyperedge embeddings, which are required for other common benchmark tasks.
Lastly, as discussed above, outputs for the problem (i.e., edge-dependent node properties) have proved useful for various applications.

% Moreover, hyperedge-dependent node embeddings, which can be generally used for other hypergraph-based tasks, 
% Second, the problem does not require global node embeddings shared by all hyperedges but require In terms of representation learning, the problem requires each model learn hyperedge-dependent node embeddings, which can be generally used for other hypergraph-based tasks, 
% Third, since the number of labels is the same as the sum of all hypergraph sizes, the problem makes a challenge in the efficiency of models; models with poor scalability fail to be run on large real-world graphs containing many hyperedges.


%In addition to its practical usefulness mentioned above.


% 5) Our contribution 2. Our model
In order to tackle the new classification task, we propose \method (\textbf{W}ithin-\textbf{H}yperedge \textbf{A}ttention \textbf{T}ran\textbf{s}former \textbf{Net}work). %based on our novel attention module, \WithinAttention. 
Most existing hypergraph neural networks do not explicitly consider edge-dependent relationships between pairs of nodes within each hyperedge.
%have not directly considered the relationships between nodes within hyperedges.
%The existing hypergraph neural networks hypergraph neural networks have not 
% Therefore, we design \WithinAttention, an attention mechanism where each node embedding is computed by attending to the other node embeddings within hyperedges. 
We design \WithinAttention, an attention mechanism where the edge-dependent embedding of each node is computed by attending to the other nodes in each hyperedge.
%the transformer where the input of queries and keys are the same from node embeddings so that pairwise relationships between nodes can be considered. 
That is, through \WithinAttention, the edge-dependent influences of nodes are  determined. % by the interactions among nodes.
Additionally, we use the centrality order of nodes within each hyperedge as the positional encoding, which makes attention in \WithinAttention even more edge-dependent, inspired by the common use of positional encodings in transformer based models.
The effectiveness of \method on the proposed task is demonstrated through extensive experiments.
% prevalence of positional encoding used in the transformer.


% restore the below
% We perform experiments on six real-world datasets from three different domains. By comparison, we demonstrate the superiority of \method over nine competitors on the proposed benchmark task. 
% %its performance. 
% Moreover, we conduct an extensive ablation study to justify the effectiveness of each component of it. We also show the usefulness of the outputs of \method in three real-world applications.

Our contributions are summarized as follows,
\begin{itemize}[leftmargin=*]
    \item \textbf{New Benchmark Task}: We propose the problem of classifying edge-dependent node labels as a new hypergraph-learning benchmark task. %Unlike general node classification tasks, node labels vary depending on hyperedges. 
    This problem is based on unique properties of hypergraphs and has proved related to real-world applications.
    \item \textbf{Effective Model}: For the problem, we design \method, a novel hypergraph neural network with attention and positional-encoding schemes that explicitly consider edge-dependent relationships between nodes.
    \item \textbf{Extensive Experiments}: Using six real-world hypergraphs, we demonstrate the superiority of \method over $9$ competitors on the proposed task. %We also conduct an extensive ablation study to justify the effectiveness of each component of it.
    We also show the usefulness of \method in three applications: ranking aggregation, node clustering, and  product-return prediction.
\end{itemize}
For reproducibility, the code and data are available at \cite{github}.

In Section~\ref{sec:related}, we review related works. In Section~\ref{sec:preliminaries}, we introduce preliminaries. In Section~\ref{sec:problem_formulation}, we describe our new benchmark task with its applications and datasets. In Section~\ref{sec:proposed_approach}, we present \method, a hypergraph neural network for this task. In Section~\ref{sec:evaluation}, we provide experimental results. Lastly, we make conclusions in Section~\ref{sec:conclusion}.
% =========================================================================
% Graph-structured data is used for representing interactions in social networks, email communication networks, and so on.  Recently, graph neural networks (GNNs) have been receiving more and more attention as a consequence of the pervasiveness of graphs. GNN learns to generate low-dimensional node, edge, or graph embeddings based on graph information. With the efforts of aggregating information well from graph structure, GNNs demonstrate powerful learning ability in various graph analytical tasks such as node classification, link prediction, and clustering. Among these tasks, Node classification is a fundamental task on graph data, which aims to classify the nodes in the graph.

% In many real-world networks, relationships are complex and go beyond pairwise associations. For example, in a co-authorship network, authors rather co-work with more than one author. Hypergraphs provide a natural representation of these groupwise interactions. To deal with the higher-order interactions in the hypergraph, several hypergraph neural networks have been proposed for representative embeddings for hypergraphs []. Their performance is usually evaluated in typical node classification same as for graphs. 

% A typical node classification problem is to classify each node into one label. In hypergraphs, however, wouldn't it be more natural that the role of nodes in a hypergraph depends on each hyperedge? For instance, in a coauthorship network, one author (node) may be the first author in any paper (hyperedge), but he is not always the first author in all other papers.

% To tackle this problem, in this paper, we define a new problem of node classification dependent on hyperedge. However, so far, the proposed models have not directly considered the relationship with the nodes they belong to the same hyperedge. Therefore, we tried to express node embeddings by reflecting the relationship with the nodes that belong together at each hyperedge. With this motivation, we propose new attention modules, \WithinAttention and \RankAttention. To evaluate the performance of the proposed \method on our new problem, we have conducted experiments on five datasets from three different domains. The results compared with other methods have demonstrated that our attention module is effective on our problem. Our ablation study further reveals the justification of our design of \method as well as our motivation.

% 3) past version - 08.08
%Unlike a typical node classification problem, which is used as an evaluation criterion for many hypergraph neural network models, in hypergraphs, the role of nodes can vary depending on the hyperedges. For example, in the co-authorship dataset, the author could be either a lead or corresponding author in a publication. Emails consist of senders, receivers, and carbon copies.  In the Q\&A platforms, the posts have questioners, answerers whose answer is adopted by the questioner, and remainders.
% Such hypergraphs contain distinct information that may not be apparent in the general hypergraph where a single label is assigned to a node.  For the publication, the roles of authors could imply the flow of collaborations, which a recent study[] % Rotabi et al. 2017
% found that conventions in preparing scholarly documentation tend to spread from the corresponding authors who are more senior to more junior authors. 
% In multi-morbidity[] where hypergraphs can represent a set of diseases observed in a population cohort, the order of diseases acquired can help the further investigation.
% Several studies have analyzed such graphs where a single node has various roles and proposed configuration model[,] or stub-matching algorithm[].

%The distinct property of our problem allows to evaluate models in a new aspect. 
% since benchmarks for hypergraph neural network learning have been quite limited yet, this new benchmark can help improve their expressive power and efficiency.
% Besides, the embeddings reflecting hyperedge-dependent node labels can be further useful in recommendation or anonymous detection. %[]

==> backup/020related.tex <==


\subsection{Hypergraph Neural Networks}
% Hypergraph neural networks are models which are developed to obtain representations of a given hypergraph.
HGNN~\cite{feng2019hypergraph} performs an ordinal graph convolution on the clique expanded graph, which is obtained by replacing each hyperedge in the input hypergraph by the complete subgraph (i.e., clique) between nodes in it.
Instead, HyperGCN~\cite{yadati2019hypergcn} does it on a graph obtained by replacing each hyperedge with an incomplete subgraph.
%where only edges that connect at least one of two mediator nodes are used for each hyperedge.

HNHN~\cite{dong2020hnhn} has two steps of message passing: (1) updating hyperedge embeddings by aggregating the embeddings of incident nodes, and (2) updating node embeddings by aggregating the  embeddings of incident hyperedges.
% With this structure, it is not equivalent to convolution in star expansion or clique expansion graph.
A non-linear function is used in both steps, and it makes the above message passing irreducible to convolution on clique-expanded graphs.
%It can also adjust the influence of each incident embedding on aggregation through hyperparameters, whereas it is fixed in HGNN and HyperGCN.

HCHA~\cite{bai2021hypergraph} computes attention weights between  pairs of incident nodes and hyperedges and use them for graph convolution.
% replaces the binary incidence matrix (i.e., a matrix that expresses the ownership of hyperedges) of HGNN with a matrix filled with attention values. 
The attention weights are computed by the dot-product between node and hyperedge embeddings, and thus they are adjusted as the model learns embeddings. However, its message passing scheme is still equivalent to graph convolution on clique expanded graphs. 
While HCHA uses the same attention weights in both directions of aggregation, HAT~\cite{hwang2021hyfer} separates them.

UniGNN~\cite{huang2021unignn} is a unified message passing framework that incorporates general graph neural networks into hypergraphs. UniGCNII, one of the variants of UniGNN, addresses the over-smoothing issue, which is common in (hyper)graph neural graphs, by extending 
%integrating a powerful graph neural network with Initial Residual Connection and Identity Mapping, 
GCNII~\cite{chen2020simple} to hypergraphs. 
% While the contributions of the incident embeddings are fixed, how much initial and previous functions affect aggregation can be controlled by the hyperparameters.

AllSet~\cite{chien2021you} is an expressive framework composed of two multiset functions. AllSet generalizes most propagation methods, including HGNN, HyperGCN, HNHN, and HCHA. Under this framework, AllSetTransformer substitutes SetTransformer~\cite{lee2019set} for the multiset function. Specifically, AllSetTrnasformer aggregates the incident embeddings by applying attention on global learnable vectors.
% Specifically, AllSetTransformer determines the attention of incident embeddings by the dot-product with the global learnable parameters.

The influence of each node may vary depending on the other nodes it interacts with within each hyperedge. However, 
most existing hypergraph neural networks do not explicitly consider edge-dependent relationships between pairs of nodes within each hyperedge.
Such relationships have been considered in
%it is not considered in the existing hypergraph neural networks. 
a few studies in a way different from ours, but none of them is directly applicable to the considered problem. % consider such interactions among nodes within hyperedges but not for hypergraph neural networks.
HyperSAGNN \cite{zhang2019hyper}, which is designed for hyperedge prediction, assumes that, in each hyperedge, the embedding of each node can be approximated by the weighted sum of the embeddings of the other nodes in the hyperedge with weights computed by pairwise attention. Thus, HyperSAGNN is trained to reduce the difference between the embedding and the weighted sum for each node in each hyperedge.
Higher-order Transformer~\cite{kim2021transformers} considers all subsets of nodes in each hyperedge\footnote{$2^e$ for each hyperedge $e\subseteq V$, where $V$ is the set of nodes} and thus computational and memory cost increases exponentially with the size of hyperedges.
Moreover, the model has been applied only to uniform hypergraphs where the size of every hyperedge is identical, and since it is built upon tensor-based representations,  it is non-trivial to directly apply it to non-uniform hypergraphs, which are considered in this paper.
%its extension to the general hypergraphs with varying sizes of hyperedges is non-trivial 
%embeddings of all subset nodes in hyperedge when computing hyperedge embedding. However, large memory is required as the size of hyperedge increases, and it is difficult to directly apply to hypergraphs with varying hyperedge sizes because it is built upon tensor-based representation of graphs.
%On the other hand, Higher-order Transformer~\cite{kim2021transformers} can consider higher-order more than pairwise relationships among nodes within hyperedges. 
%Since being modeled for uniform hypergraphs, however, its extension to the general hypergraphs with varying sizes of hyperedges is non-trivial.

% ====================================================================================================================
\subsection{Positional Encodings} \label{sec:pe}
%GNNs cannot distinguish two different nodes with the same neighborhood structure if node attributes are the same. 
%Formally speaking, the representational capacity of the model is at most as powerful as the WL test~\cite{xu2018powerful, morris2019weisfeiler, weisfeiler1968reduction}.
Graph neural networks (GNNs) have difficulty discriminating the positions of different nodes if they have similar local structures~\cite{you2019position}. Various positional encodings for graphs have been proposed in order to improve the representation power. Such positional encodings, which we call \textit{absolute positional encodings}, are often added or concatenated to the node features, and they are based on random discriminating features~\cite{murphy2019relational,sato2021random,kipf2016variational,zhang2018link,hamilton2017inductive}, Weisfeiler–Lehman~\cite{zhang2020graph}, Laplacian Eigenvectors~\cite{dwivedi2020generalization,belkin2003laplacian,dwivedi2020benchmarking,kreuzer2021rethinking}, random walk~\cite{li2020distance,dwivedi2021graph,ahmadi2020memory}, etc. 
%On the other hand, new graph neural networks are developed for capturing nodes’ positional information~\cite{you2019position,wang2022equivariant}.
Alternatively, GNNs that are able to capture positional information of nodes~\cite{you2019position,wang2022equivariant} can be used.

% As transformer models are commonly provided explicit positional information of each word in Natural Language Processing (NLP), the positional encoding methods are also employed by Transformer based GNNs. 
In Natural Language Processing, Transformer models are commonly provided explicit positional information about each word. Motivated by this, several Transformer-based GNNs are given external positional information for each node.
Graph Transformer~\cite{dwivedi2020generalization} and SAN~\cite{kreuzer2021rethinking} use Laplacian eigenvectors. Graph-Bert~\cite{zhang2020graph} represents nodes differently through the Weisfeiler algorithm~\cite{niepert2016learning}. Graphormer~\cite{ying2021transformers} adds global degree centrality to node features so that its self-attention module can capture both semantic correlations among nodes and the difference in their centrality.
It supports the effectiveness of employing node centrality, which we also use in a different way for positional encoding in our attention mechanism.

%Since we also use  for positional encoding in our attention mechanism, 

Besides the absolute positional encodings, \textit{relative positional encodings}~\cite{raffel2020exploring, shaw2018self} are also used in Transformer-based GNNs to affect attention mechanisms based on the relative distance between nodes (e.g., between a query and a key).
The relative distance can be computed based on positive definite kernels on graphs~\cite{mialon2021graphit}, learnable positional embeddings~\cite{ma2021graph}, shortest path distance~\cite{park2022grpe, ying2021transformers}, multi-step transition probability~\cite{zhao2021gophormer}, etc.
% Since we use the node centrality as a positional encoding for our attention mechanism, Graphormer is most related to our work. Besides the absolute positional encodings, a \textit{relative positional encoding} is also used in Transformer~\cite{raffel2020exploring, shaw2018self}. It gives a bias to the self-attention calculation with the relative positional difference between the query and key. The relative positional difference can be determined in the graph by the positive definite kernels on graphs~\cite{mialon2021graphit}, learnable positional embeddings~\cite{ma2021graph}, shortest path distance~\cite{park2022grpe, ying2021transformers}, or reachable probabilities of higher-order~\cite{zhao2021gophormer}.





% Previous -----------------------------------------------------------------------------------------------
% HyperGCN ... % does it on a graph converted from a hypergraph by replacing each hyperedge with only edges connected to two specific mediators in it so that less number of edges are used than a clique.
%UniGCNII~\cite{huang2021unignn}, which also has a two-step message passing like HNHN and considers the first layer value in updating step, is presented to solve the problem of over-smoothing. The contribution of the first layer value compared to the value obtained by aggregation is determined by the hyperparameter.
% UniGNN~\cite{huang2021unignn} is a unified framework for message passing which makes it easier to incorporate general graph neural networks into hypergraphs. UniGCNII, one of the variants of UniGNN, even solves over-smoothing phenomenon by incorporating a powerful graph neural network with Initial Residual Connection and Identity Mapping, GCNII~\cite{chen2020simple}. In UniGCNII, the contributions of incident embeddings are fixed but how much inject the initial features and previous features are controlled by the hyperparameters.
%AllSet~\cite{chien2021you} has two steps of message passing like HNHN but allows the contribution of embeddings to be learned in the update phase. Specifically, the contribution of the embeddings is determined by the dot-product between the corresponding embeddings and the global learnable parameters when aggregation of each step occurs. Here, the global learnable parameter is that there is only one in common at each step, not personally present at each node or hyperedge being updated.
% AllSet~\cite{chien2021you} is an expressive framework composed of two multiset functions which can cover most propagation methods including HGNN, HyperGCN, HNHN, and HCHA. In this framework, AllSetTransformer is inspired by Set Transformer~\cite{lee2019set}. Specifically, AllSetTransformer determines the contribution of incident embeddings by the dot-product between the corresponding embeddings and the global learnable parameters. Here, the global learnable parameter does not exist personally on each node or hyperedge being updated, but exists in common for all nodes or hyperedges.
%However, the existing hypergraph neural networks have not determined the contribution of node embeddings by pairwise attention within them. Even though Hyper-SAGNN~\cite{zhang2019hyper} considers this, it is designed for the purpose of hyperedge prediction. To be specific, the possibility of a hyperedge is determined by how similar the embeddings of one node are to the weighted sum of embeddings of other nodes where the weights are obtained by pairwise dot-product between embeddings of nodes in this hyperedge. Such a structure is not suitable for node classification, so we would like to consider such a contribution in a new node classification.
% Hyper-SAGNN~\cite{zhang2019hyper} considers such a relationship for hyperedge prediction. It learns the weights of node embeddings in order that the static embedding of one node which remains the same regardless of the hyperedge can be made by the weighted sum of the embeddings of the other nodes in the real hyperedge. Thus, it is different from our goal of learning the weights to reflect the pairwise relationships within hyperedges and affect the contributions of nodes to hyperedges in the message passing.
% On the other hand, Higher-order Transformer~\cite{kim2021transformers} can consider higher-order more than pairwise relationships among nodes within hyperedges. However, it is modeled for uniform hypergraphs, so its extension to the general hypergraphs with varying sizes of hyperedges is non-trivial.
% Since it is implemented by tensors and the number of basis grows rapidly with the hyperedge size, however, it is hard to be applied to general hypergraphs with varying sizes of hyperedges.
% Therefore, it learns the static embedding of one node which remains the same regardless of the hyperedge to be similar to the weighted sum of the other node embeddings within the real hyperedge. Thus, it differs from our goal of determining the contributions by considering the relationship between nodes in the message passing.

%In addition, Higher-order Transformer~\cite{kim2021transformers} is proposed to model higher-order relations of nodes within hyperedges. However, since this model is only applicable to the uniform hypergraph (i.e., hypergraph where the size of every hyperedge is identical), its extension to the general hypergraph, which may have an arbitrary size hyperedge, is non-trivial.

% Previous -----------------------------------------------------------------------------------------------
%Recent studies showed that the representation power of GNNs is bounded by the 1-WL test~\cite{xu2018powerful, morris2019weisfeiler, weisfeiler1968reduction}. 
% Various positional encodings have been proposed to improve the representation power of GNNs which is bounded by 1-WL test~\cite{xu2018powerful, morris2019weisfeiler, weisfeiler1968reduction} and their effectiveness is demonstrated for prediction tasks~\cite{srinivasan2019equivalence,cui2021positional}. 
% In NLP, transformer models are commonly provided an explicit positional information of each word, termed as a positional encoding~\cite{vaswani2017attention, raffel2020exploring, shaw2018self}.
% Therefore, several positional encodings for the graph neural networks have been proposed to integrate graph structural information into the transformer architecture.
% One of the type is \textit{absolute encoding}, where the positional encoding is added or concatenated to the input node features. Examples of methods consider Weisfeiler–Lehman~\cite{zhang2020graph}, Laplacian Eigenvectors~\cite{dwivedi2020generalization,belkin2003laplacian,dwivedi2020benchmarking,kreuzer2021rethinking}, random walk~\cite{li2020distance,dwivedi2021graph} and centrality~\cite{ying2021transformers}. 
% The other type is \textit{relative encoding}~\cite{raffel2020exploring, shaw2018self}. This strategy gives bias to the self-attention calculation with the relative positional difference between the query and key nodes. The relative positional difference is determined by the positive definite kernels on graphs~\cite{mialon2021graphit}, learnable positional embeddings~\cite{ma2021graph}, shortest path distance~\cite{park2022grpe} or reachable probabilities of higher-order~\cite{zhao2021gophormer}.

==> backup/040preliminaries.tex <==
In this section, we define the concepts necessary to describe our method. The frequently-used symbols are summarized in Table~\ref{tab:notations}. % We first define a hypergraph and then an attention mechanism.

\subsection{Hypergraph}
A hypergraph $\Glong$ consists of a set of nodes $\SV =\{v_1, \ldots,v_N\}$ and a set of hyperedges $\SE = \{e_1, \ldots,e_M\} \subseteq2^{\SV}$. Each hyperedge $e\in \SE$ is a non-empty subset of $\SV$. 
We use $\mathcal{N}_{v} =\{e \in \SE :  v \in e\}$ to denote the set of hyperedges incident to the node $v$, i.e., the set of hyperedges that contain $v$.
%Similarly, we use $\mathcal{N}_{e} = \{ v \in \SV |  v \in e\}$ to denote the set of nodes incident to the node $v$, i.e., the set of hyperedges that contain $v$.
%\textit{incident nodes} of a hyperedge $e$ indicate a set of nodes within the hyperedge $e$ and they are denoted as 


\subsection{Attention}
\smallsection{Scaled Dot-Product Attention}
For $n_q$ query vectors $\mathbf{Q} \in \mathbb{R}^{n_q \times d_k}$ and $n_k$ key-value vector pairs $\mathbf{K} \in \mathbb{R}^{n_k \times d_k}$ and $\mathbf{V} \in \mathbb{R}^{n_k \times d_v}$, the scaled dot-product attention module computes the weighted sum of values as follows:
\begin{equation*}
    Attention(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = softmax(\frac{\mathbf{QK}^\top}{\sqrt{d_k}})\mathbf{V},
\end{equation*}
where $\sqrt{d_k}$ is typically used to avoid exploding gradients~\cite{vaswani2017attention}.
Note that the more similar a query vector and a key vector are (i.e., the larger their dot product is), the larger the corresponding weight is. % query is expressed as a weighted sum of values with the more weights on that key:
%Here, $\sqrt{d_k}$ is used to prevent the results of the dot product from becoming too large to increaseing the gradient value as mentioned in ~\cite{vaswani2017attention}.

\smallsection{Multihead Attention}
A multihead attention module~\cite{vaswani2017attention} of dimension $d_k$ consists of $h$ attention modules of dimension $d_k/h$, whose outputs are concatenated, for the final output as follows:
% Instead of computing attention on entire $d_k$ dimensions,  divides it into $h$ attentions each of which is computed on $d_k/h$ dimensions.
% Each attention is processed in parallel so that it takes a similar amount of time as the single-head attention.
% The final output is obtained by concatenating the outputs of the $h$ attentions as follows:
% Therefore, different attention can be considered depending on the position of the output.
% Instead of a single attention with the entire dimension of $Q$ and $K$, i.e. $d_k$, Multihead attention first splits $Q, K$ and $V$ into $h$ different $Q_{i}, K_{i}$ and $V_{i}$ which dimension is $d_k / h, d_k / h$ and $d_v / h$ respectively. An attention module is applied to each of $h$ different positions of the inputs and then these outputs are concatenated into a final output.
\begin{equation*}
    MultiheadAttention(\mathbf{Q,K,V}) = Concat(\mathbf{O}_{1}, \cdots, \mathbf{O}_{h})\mathbf{W^{O}},
\end{equation*}
where $\mathbf{O}_i = Attention(\mathbf{Q}_i, \mathbf{K}_i, \mathbf{V}_i) = Attention(\mathbf{Q} \mathbf{W}^\mathbf{Q}_i, \mathbf{K} \mathbf{W}^\mathbf{K}_i, \mathbf{V} \mathbf{W}^\mathbf{V}_i)$.
% $\mathbf{Q}\in \mathbb{R}^{n_q \times d_Q}$, $\mathbf{K}\in \mathbb{R}^{n_k \times d_K}$, and $\mathbf{V}\in \mathbb{R}^{n_k \times d_V}$ 
That is,
$\mathbf{Q}$, $\mathbf{K}$, and $\mathbf{V}$ 
are mapped into subspaces 
$\mathbf{Q}_i\in \mathbb{R}^{n_q \times (d_k/h)}$, $\mathbf{K}_i\in \mathbb{R}^{n_k \times (d_k/h)}$, and $\mathbf{V}_i\in \mathbb{R}^{n_k \times (d_v/h)}$, respectively, by learnable parameters $\mathbf{W}^\mathbf{Q}_i\in \mathbb{R}^{d_k \times (d_k/h)}$ ,$\mathbf{W}^\mathbf{K}_i\in \mathbb{R}^{d_k \times (d_k/h)}$, and $\mathbf{W}^\mathbf{V}_i\in \mathbb{R}^{d_v \times (d_v/h)}$.
In our experiments,
the matrix $\mathbf{W}^\mathbf{O} \in \mathbb{R}^{d_v \times d_v}$ is fixed to the identity matrix, and the number of heads $h$ is set to $4$. %heads in our experiments.
% Here, the dimension of $\mathbf{Q, K,}$ and $\mathbf{V} $ is $d^{Q}, d^{K}$, and $\mathbf{d^{V}}$ respectively.
% $\mathbf{Q, K}$, and $\mathbf{V}$ are mapped to $h$ separate subspaces by learnable parameters $\mathbf{W^{Q}_{i} \in \mathbb{R}}^{d^{Q} \times d^{Q}_{i}}$, $\mathbf{W^{K}_{i}} \in \mathbb{R}^{d^{K} \times d^{K}_{i}}$ and $\mathbf{W^{V}_{i}} \in \mathbb{R}^{d^{V} \times d^{V}_{i}}$. 
% Typically, $d^{Q}_{i} = d^{K}_{i} = d_k / h$ and $d^{V}_{i} = d_v / h$.
% Finally $\mathbf{O} \in \mathbb{R}^{d_v \times d}$ updates the $d_v$ dimensional concatenated outputs into the final output dimension $d$. And we employ $h = 4$ heads in our experiments.


\begin{table}[t!]
    \vspace{-3mm}
	\caption{\label{tab:notations}Frequently-used symbols.}
	\scalebox{0.84}{
		\begin{tabular}{c|l}
			\toprule
			\textbf{Notation} & \textbf{Definition}\\
			\midrule
			% graph
			$\Glong$ & a hypergraph with nodes $\SV$ and hyperedges $\SE$\\
		%	$\mathcal{Y}_{(\SV, \SE)}$ & edge-dependent node labels\\
			$N, M$ & the number of nodes and hyperedges \\
			$C$ & the number of (unique) edge-dependent node labels \\
			\midrule
			% scalar
			$v, e$ & a node $v \in \SV$ and a hyperedge $e \in \SE$ \\
			$y_{v, e}$ & the edge-dependent label of node $v$ in hyperedge $e$. \\
			$\mathcal{N}_{v}$ & the set of hyperedges incident to a node $v$ \\
			\midrule
			$l, m$ & the number of layers and inducing points\\
% 			$m$ & the number of inducing points\\
			$d_l$ & the hidden dimension at $l$-th layer \\
			$d_f$ & the dimension of \PE \\
			\midrule
			% matrix
			$\mathbf{F}$ & a node centrality feature matrix \\
			$\mathbf{I}_{w}$ & trainable inducing points in \WithinAttention \\
			$\mathbf{X^{(l)}, H^{(l)}}$ & a node/hyperedge embedding matrix at layer $l$ \\
% 			$H^{(l)}$ & an hyperedge feature matrix at layer $l$ \\
% 			$V_e, R_e$ & the feature and relative rankings of the incident nodes of a hyperedge $e$ \\
% 			$E_v, R_v$ & the features and relative rankings of the incident hyperedges of a node $v$ \\
            $\mathbf{V_e}, \mathbf{E_v}$  & an embedding matrix of $e$ and $\mathcal{N}_{v}$ \\
            % $R_v, R_e$ & the relative rankings among $\mathcal{N}_{v}$ and $\mathcal{N}_{e}$ \\
			\bottomrule
		\end{tabular}}
\end{table}

\smallsection{Multihead Attention Block}
We use the multihead attention block (MAB)~\cite{vaswani2017attention} as a component of our model.
It consists of a multihead attention module, a feed forward layer, residual connection~\cite{he2016deep}, and layer normalization~\cite{ba2016layer} as follows:
\begin{equation*}
    MAB(\mathbf{Q, K}) = LayerNorm(\mathbf{H} + FeedForward(\mathbf{H}))),
\end{equation*}
where $\mathbf{H} = LayerNorm(\mathbf{Q} + MultiheadAttention(\mathbf{Q,K,K}))$.
Note that the feed forward layer does not change the dimensionality of the input matrix.

% Linear attention scheme with inducing points
\smallsection{Attention with Inducing Points} \label{attwinducing} The scaled dot-product attention module requires all-pair dot-products between the query vectors and key vectors, and thus its time complexity quadratic, specifically $O(n_q n_k)$. %quadratic with the number $n_q$ of queries and the number $n_k$ of keys.
SetTransformer~\cite{lee2019set} introduces an attention scheme which reduces the complexity to be linear.
With $m \ll \min(n_q, n_k)$ trainable inducing points, denoted by $I$, the all-pair dot-product is approximated by $\MultiheadAtt(\mathbf{Q}, \MultiheadAtt(\mathbf{I, K}))$ whose time complexity is $O(m(n_q + n_k))$.
We adopt this strategy in our model for efficiency.

% This reduces a computation of the scaled dot-product between $\mathbf{Q}$ and $\mathbf{K}$ into a computation of scaled dot-product between $\mathbf{Q}$ and $\mathbf{I}$ and between $\mathbf{K}$ and $\mathbf{I}$, which becomes $O(m n_q)+O(m n_k)=O(n_q + n_k)$.


==> backup/050problem_formulation.tex <==
In this section, we define our problem and present six real-world datasets for it. Then, we introduce three applications of the problem.

\subsection{Problem Formulation}

% In this section, we formulate a new problem we are going to solve.
In classical node classification, a single label is assigned to every node. 
% \red{Formally, let label space of each node as $Y=\{1, 2, \cdots , |Y|\}$ and denotes $\mathcal{Y}_{prev}(v_{i})$ a label of a node $v_{i}$ on classical node classification where a function $\mathcal{Y}_{prev} : \SV \mapsto Y$ is a bijective function (i.e., every input corresponds to only one output).} 
However, in hypergraphs, the labels of nodes can be different depending on hyperedges that they are included in. For example, in a  co-authorship hypergraph, a researcher can be classified into the first, last and middle authors, and the position may change according to  publications. 
Note that such edge-dependent node labels are unique in hypergraphs, and especially they disappear in clique-expanded graphs, which are the result of direct simplification of hypergraphs into ordinary graphs.
Based on this unique charcteristic of hypergraphs, we propose a new hypergraph-learning benchmark task, which we refer to edge-dependent node classification.  
The problem is formalized in Problem~\ref{problem}.
% Formally, let a new edge-dependent node labeling function as $ f : \mathcal{V} \times \mathcal{E} \mapsto \{1,2, \cdots, C \}$ which is a bijective function either. From this setting, we define our main problem as follows:

\begin{pro}[Edge-dependent node classification]\label{problem}
Given (a) a hypergraph $\SG = (\SV, \SE)$, (b) edge-dependent node labels %$\mathcal{Y}_{\SE'}  = \{ y_{v, e} : v \in e, e \in \SE' \}$ where $\SE' \subset \SE$,
in $\SE' \subset \SE$ (i.e., $y_{v, e}, \forall v \in e, \forall e \in \SE'$),
and optionally (c) a node feature matrix $\mathbf{X}$,
the problem is to predict the unknown edge-dependent node labels in $\SE \setminus \SE'$ (i.e.,  $y_{v, e}, \forall v \in e, \forall e \in \SE \setminus \SE'$).
\end{pro}
\noindent Refer to Section~\ref{sec:intro} for a further discussion why this problem is a proper benchmark task for hypergraph neural networks

% \begin{pro}
% Given a hypergraph $\SG = (\SV, \SE)$ with node initial feature matrix $\mathbf{X}$ and partial edge-dependent node labels $\mathcal{Y}_{(\SV, \SE')}  = \{f(v, e) : v \in e, e \in \SE\}$ where $\SE' \subseteq \SE$, the problem is to predict the unknown edge-dependent node labels, formally $\mathcal{Y}_{(\SV, \SE'')}$ where $\SE'' = \SE \setminus \SE''$.
% \end{pro}

% ==================================================================================================
% formulation
% Here, we define set of every node's label as $Y_{(\SV, \SE)} = \{\mathcal{Y}(v, e) : v \in e, e \in \SE\}$. 
% Given a hypergraph $G = (\SV, \SE)$ where $\SV$ is the set of nodes and $\SE=\{\SE_{train},\SE_{valid},\SE_{test}\}$ is the set of hyperedges splitted into train/valid/test and edge-dependent node labels $\SL = \{ \SL_{train} = l_{v,e} \forall v \in e, e \in \SE_{train}, \SL_{valid}, \SL_{test} \}$, the goal of hypergraph neural networks is to learn effective node and hyperedge embeddings that are well classified unknown labels $\SL_{valid}$ / $\SL_{test}$ based on the neighborhood structure and the given labels $\SL_{train}$

% Task Framework
% We formulate our new task as \ref{problem}. The given data is a hypergraph where hyperedges are splitted into train/valid/test sets and the labels are assigned to the node and hyperedge pairs. The embeddings of both nodes and hyperedges are obtained from Hypergraph Neural Network on the given hypergraph. Then, for the hyperedges in the training set and all nodes included in these hyperedges, the probability distribution of their labels are decided by passing the concatenation of node and hyperedge embedding into the feed forward layer and softmax layer. By the known labels for the training set, the Hypergraph Neural Networks are trained with the Cross Entropy Loss. After training the Hypergraph Neural Networks, they are evaluated by how accurately they predict the labels in the valid or test set. 
% \noindent\fbox{%
%     \parbox{0.98\columnwidth}{%
%     \vspace{-2mm}
% \begin{problem}[Edge-Dependent Node Classification on a Hypergraph \label{problem}] \
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Given}: \\ 
%     a hypergraph $G = (\SV, \SE)$ where $\SE=\{\SE_{train},\SE_{valid},\SE_{test}\}$ and $\SL=\{ l_{v,e} \forall v \in e, e \in \SE \}$
%     \item \textbf{Learning}: \\ 
%     $X, H \leftarrow$ HypergraphNeuralNetwork($G$) \\
%     Train HypergraphNeuralNetwork by CrossEntropyLoss( SoftMax(FF($X_{v} || H_{e}$)), $l_{v,e}$) for $v \in e, e \in \SE_{train}$
%     \item \textbf{Inference}: \\ 
%     Predict $\hat{l}_{v,e} \leftarrow $ ArgMax(SoftMax(FF($X_{v} || H_{e}$))) for $v \in e, e \in \SE_{valid/test}$
% \end{itemize}
% \end{problem}
%         \vspace{-2mm}
%         }%
%     }
%Formally, given a hypergraph $G = (\SV, \SE)$ and a set of node labels $Y$, each pair of node and hyperedge where it is included has one unique label $y_{(v,e)} \in Y$. As typical node classification tasks, only part of pairs of nodes and hyperedges have known labels during training. Let denote these pairs as $VE_{L}$. The goal of this problem is to learn a graph-based mapping function $f_{\theta} : \{v,e,G\} \rightarrow \{1,2, ... ,|Y|\}$ with $VE_{L}$ and then $f_{\theta}$ can map each unlabeled pair of nodes and hyperedges to one label.

% ==================================================================================================
\subsection{Benchmark Datasets}\label{benchmark_dataset}



We introduce six real-world datasets for our new benchmark task, they are from $3$ different domains.
\begin{itemize}[leftmargin=*]
    \item \textbf{Co-authorship} (DBLP~\cite{Swati2016dblp} and AMinerAuthor\footnote{https://www.aminer.org/aminernetwork}): Each hyperedge indicates a publication, and the nodes in it correspond to the authors of the publication. Edge-dependent node labels indicate the orders of authors (first, last, or others) in each publication. 
    \item \textbf{Email} (Enron\footnote{https://www.cs.cmu.edu/~enron/} and Eu~\cite{paranjape2017motifs}): Each hyperedge represents an email, and the nodes in it are people involved in the email. They are the sender, the receivers, or those CC'ed, which are the three edge-dependent labels. 
    %separated by the sender, receiver, and cc (carbon copy).
    \item \textbf{StackOverflow} (Biology\footnote{\label{footnote:stack}https://archive.org/download/stackexchange} and Physics~\footref{footnote:stack}): Each hyperedge represents a post, and the nodes in it represent the users who contribute to this post. Nodes are the questioner, the answerer adopted by the questioner, or the other answerers, which are the three edge-dependent labels.
\end{itemize}
The properties of the datasets and how they are preprocessed are described in detail in Appendix~\ref{appendix:data}.

% ==================================================================================================



\subsection{Applications}\label{benchmark_application}
A hypergraph neural network trained for our problem can predict unknown edge-dependent node labels in the input hypergraph. Edge-dependent node labels  give information about the influence of nodes within each hyperedge, and leveraging this information has proved useful in a variety of applications.
% The usefulness of knowing different labels of vertices within hyperedges is demonstrated in various applications. 

% [Structure]
% 1. explain about task + usefulness in real-life
% 2. what edge-dependent node label means
% 3. How these weights are used in algorithm -> good performance + citation



\smallsection{Ranking Aggregation}
The ranking aggregation task is to predict the overall ranking when only the rankings are partially known. For example, in a multiplayer game, participants compete for points, and their rankings are determined for each match.
%All players can't compete simultaneously in one match, but if expecting the rankings of all players well, a more exciting game can be made by matching competitive players. 
If we infer the global ranking of players from their local (each game) ranking, the game could be more exciting by matching competitive players. 
%However, it is practically impossible for too many players to play in one match simultaneously, so the exact overall ranking is difficult to know.
This task can be solved based on a hypergraph where (a) each node is a player, (b) each hyperedge is a match, (c) and the participants of a match are labeled based on their contribution levels during the match, as described in ~\cite{chitra2019random}. 
% The players can be ranked by the stationary distributions from the random walks with a higher probability of visiting nodes with higher level within the hyperedge as described in ~\cite{chitra2019random}.
%, and this showed high accuracy in overall player ranking predictions. Here, the edge-dependent node labeling by the rankings of participants in each match can be leveraged for weighting.

\smallsection{Clustering}
Clustering is the process of grouping similar elements, and it is widely-used for data analysis. 
Hayashi et al. \cite{hayashi2020hypergraph} designed a node clustering capable of exploiting edge-dependent node weights and showed that it produces high-quality clusters for real-world hypergraphs.
Edge-dependent node labels inferred for Problem~\ref{problem} can be transformed into weights for node clustering.
For example, in a coauthorship dataset, authors (nodes) can be weighted according to their position (e.g., first, last, or others) in each publication (hyperedge) to be better clustered. % publications can be grouped by their submitted conference.
% It can also be used to find similar diseases by modeling hypergraphs where nodes are diseases, hyperedges are genes, and nodes are divided by their association to disease which would be computed by "Gene Disease Association" (GDA) scores\footnote{https://www.disgenet.org/}.



\smallsection{Product Return Prediction}
In E-commerce, the prediction of the customer's intention to return products is demanded for E-tailers to take proactive actions.
Li et al.~\cite{li2018tail} showed that
the product return probability of each target basket can be quite accurately estimated using  hypergraphs where nodes are baskets and hyperedges are products. Specifically, they labeled baskets (nodes) according to the number of each product (hyperedge) that it contains, 
% Because products are more likely to be returned if the buyer purchases multiple items of the same product in different colors or sizes, the labels can give information about whether or not multiple items are purchased.
and showed that
the labels are informative in predicting product returns. For example, multiple purchases of the same product in one basket often correspond to the purchases of the same product with different colors or sizes, and thus one or more products in the basket are likely to be returned.

% \smallsection{Anomaly Detection}
% Anomaly in networks could corrupt the quality of recommendations or manipulate the centralities, so detecting anomalous hyperedges in real-time is useful. 
% The real-time processing of streaming hyperedges needs hypergraphs to be summarized. After combining nodes into a supernode and labeling supernodes with their occurences in each hyperedge, a hypergraph can be summarized. Based on the proximity between supernodes tracked by random walks where supernodes with higher occurrences are visited more at each hyperedge, detecting the unexpected high proximity can identify anomalous hyperedges as described in ~\cite{lee2022hashnwalk}.

% Previous =========================================================
% \vspace{0.5mm}
% \noindent\fbox{%
%         \parbox{0.98\columnwidth}{%
%         \vspace{-2mm}
% \begin{problem}[Edge-Dependent Node Classification\label{problem}] \
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Given}: - a hypergraph $G = (\SV, \SE)$
%     \item[] \qquad \quad - a label set $Y = \{ y_{(v,e)} | \forall v \in e, \forall e \in \SE \}$
%     \item[] \qquad \quad - train/test split $X_{train}, X_{test} \in \SE$ 
%     %such that $X_{train} \cap X_{test} = \o$ and $X_{train} \cup X_{test} = \SE$
%     \item \textbf{Train}: make embeddings of node and hyperedge based on $G$ and update them to predict accurately $Y_{train} = \{y_{(v,e)} |\forall v \in e, \forall e \in X_{train} \}$ 
%     \item \textbf{Evaluate}: predict $Y_{test} = \{y_{(v,e)} |\forall v \in e, \forall e \in X_{test} \}$ by using embeddings of node and hyperedge from $G$
% \end{itemize}
% \end{problem}
%         \vspace{-2mm}
%         }%
%     }
% \vspace{0.5mm}

% -------------------------------
% Clustering is grouping similar elements and is useful in the analysis of data. 
% It is shown that the clustering methods designed with the incidence matrices and the Laplacians of hypergraphs with edge-dependent node labels produce high-quality clusters~\cite{zhu2022bhypergraphs, hayashi2020hypergraph}.
% For example, it showed performance on classifying documents by categories in hypergraphs where documents and words are taken as nodes and hyperedges respectively and corresponding edge-dependent node labels are the tf-idf values, and finding similar diseases by modeling hypergraphs in which nodes are diseases, genes are hyperedges, and  edge-dependent node labels are "Gene Disease Association" (GDA) score taken from DisGeNET\footnote{https://www.disgenet.org/}. Additionally, in our experiment, we experiment classifying publications according to conferences in our DBLP dataset. 
% Also, the penalty of splitting a hyperedge reflecting the EDVW show the effectiveness in the binary classification of nodes~\cite{zhu2022ahypergraph}.

% -------------------------------
% Clustering is a grouping of similar elements and is useful for data analysis. 
% A clustering method designed with the Laplacians of hypergraphs with different weights for nodes depending on the hyperedge produces high-quality clusters~\cite{zhu2022bhypergraphs, hayashi2020hypergraph}.
% For example, it showed the ability to categorize documents by using hypergraphs where nodes and hyperedges are documents and words, and nodes are weighted by tf-idf values.
% It also succeeded in finding similar diseases by modeling hypergraphs where nodes are diseases, hyperedges are genes, and the weights of nodes depending on hyperedges indicate "Gene Disease Association" (GDA) scores taken from DisGeNET\footnote{https://www.disgenet.org/}. 
% In both of the above cases, identifying edge-dependent node labels corresponding to ranking by node weight within the hyperedge can be expected to have the same effect. Actually, we were able to confirm from experiments that it was good at classifying publications according to conferences in our DBLP dataset.

% -------------------------------
% In E-commerce, the prediction of the customer's intention to return is demanded for E-tailers to take proactive actions. 
% The return prediction of a target basket based on similar historical baskets from a local graph cut in hypergraphs showed effectiveness~\cite{li2018tail}. The nodes and hyperedges in the hypergraphs represent shopping baskets and products respectively and the weights of the basket are used to represent the number of products in the basket. 
% Edge-dependent node labels can also be applied to indicate the count of products in the baskets.

% By constructing hypergraphs where nodes, hyperedges, and EDVW correspond to shopping baskets, products and the counts of the product in the basket respectively, cut conductance is defined by reflecting the EDVW. By obtaining the local cluster with the minimum cut conductance which consists of a target basket and its similar baskets, this task aims to predict the return probability of the target basket and which products in the basket will be returned. The success in product return prediction can help for e-tailers to take proactive actions for decreasing return intention~\cite{li2018tail}.

% -------------------------------
% The measuring anomalousness of a hyperedge by using the proximity between nodes which is estimated by random walks on hypergraphs with EDVW is successful in real-world hypergraphs~\cite{lee2022hashnwalk}.


==> backup/060proposed_approach.tex <==
\begin{figure*}
    \vspace{-2mm}
    \begin{minipage}{0.51\linewidth}\label{fig:ouratt}
        \includegraphics[width=1.0\linewidth]{FIG/model/attention3.jpg}
        \subcaption{Illustration of \WithinAttention}
    \end{minipage}
    \begin{minipage}{0.48\linewidth}\label{fig:ourmodel}
         \includegraphics[width=1.0\linewidth]{FIG/model/model3.jpg}
         \vspace{0.1cm}
         \subcaption{Architecture of \method in Aggregation at Hyperedge}
    \end{minipage}
    % \vspace{-0.1cm}
    \caption{(a) In the given hypergraph, which consists of $e_1 = \{ v_1, v_2, v_4\}, e_2 = \{ v_2, v_3, v_4, v_5 \}$, \WithinAttention is applied to $e_1$ and $e_2$ independently. Even though the input feature of the node $v_2$ is same, the output is different within $e_1$ and $e_2$. The inducing points for efficiently calculating pairwise interactions are used globally. (b) The embeddings of the nodes in the target hyperedge are fed into \WithinAttention after \PE is added to each. Then, the outputs (i.e., edge-dependent node embeddings) are aggregated to update the embedding of the target hyperedge.}
\end{figure*}
% \begin{figure}\label{fig:ourmodel}
%     \includegraphics[width=1.05\linewidth]{FIG/model/model2.jpg}
%     \caption{\method Structure}
% \end{figure}
% \begin{figure}\label{fig:ouratt}
%     \includegraphics[width=1.05\linewidth]{FIG/model/attention2.jpg}
%     \caption{\WithinAttention Structure}
% \end{figure}


% ------------------------------------------------------------------------



In this section, we propose \method (\textbf{W}ithin-\textbf{H}yperedge \textbf{A}ttention \textbf{T}ran\textbf{s}former \textbf{Net}work), a hypergraph neural network for edge-dependent node classification.
Each layer of \method conducts two steps of message passing: (1) updating hyperedge embeddings by aggregating node embeddings which belong to it, and (2) updating node embeddings by aggregating hyperedge embeddings which include the corresponding node.
The message passing is composed of an attention module, which considers edge-dependent (or node-dependent)
interactions among adjacent nodes (or hyperedges), and an aggregation module for aggregating incident embeddings into one with adequate weights.
These two modules are called \WithinAttention and \aggregation, respectively.
% Each layer of \method updates the embeddings of all nodes and hyperedges through \WithinAttention and \aggregation.
% Given a set of incident nodes (or hyperedges),  \WithinAttention updates their embeddings by considering pairwise or higher interactions through an attention mechanism.

% The embeddings of both nodes and hyperedges are made by our \method and then their concatenation is fed into a softmax layer to predict the node labels depending on the corresponding hyperedge.
% Unlike the conventional node label prediction tasks, in our problem, node labels changes according to hyperedges. Thus both node and hyperedge embeddings are considered together in prediction.

We first discuss intuitions behind the \WithinAttention module in Section~\ref{method:motivation} and describe its structure in Section~\ref{method:attention}. Then, we describe the \aggregation module in Section~\ref{method:aggregation}. After that, we present the overall architecture of \method in Section~\ref{method:overall}. Lastly, we analyze its time complexity in Section~\ref{method:analysis} and specify how it is different from existing hypergraph neural networks in Section~\ref{method:comp}. Since the structures of the message passing in both directions (i.e., nodes to hyperedges and hyperedges to nodes) are symmetric, we focus on the message passing from nodes to hyperedges. % for the simplicity of the explanation. 


% ------------------------------------------------------------------------
\subsection{Motivations}\label{method:motivation}
% Relative Position
What characterizes our problem is that the node labels change depending on hyperedges. In other words, the influence of a node would be affected by the relationship with the other nodes included together. For example, if one professor co-author a paper only with students, it is likely that she is the last author of the paper. However, if she co-authors a paper with other professors, then the probability of her being the last author of the paper is relatively low.



% Ranking
In addition, we expect that edge-dependent node labels are closely related to the relative positions of nodes within each hyperedge, which can be measured, for example, by  centrality relative to the other nodes in each hyperedge. For example, in co-authorship hypergraphs, degree centrality indicates the number of papers authored by each researcher.
It is likely that the researcher with a centrality higher than the other co-authors of a paper is the last author of the paper.

% Therefore, it is more likely that the author with the highest degree among co-authors is a corresponding author.

% Not considered in most of other models
However, most existing hypergraph neural networks do not explicitly consider the edge-dependent relations between pairs of nodes during message passing. Thus, we devise \WithinAttention, where edge-dependent embedding of each node is computed by attending to the other nodes in each hyperedge.
We also use the centrality order of nodes within each hyperedge as the positional encoding, which makes attention in \WithinAttention even more edge-dependent. % The use of positional encodings is inspired by the common use of positional encodings in transformer based models.
% Furthermore, following the practice of using positional encoding for transformers in NLP, we are motivated to use node centralities as positional encodings.
% considered the relation between nodes within the hyperedge. 
% Thus we are motivated to get a node representation by utilizing the pairwise interactions among nodes within the hyperedge. To this end, we devise our \WithinAttention which allows each node to attend to other nodes in the incident hyperedges.
%which uses attentions between nodes that belong together.

% ------------------------------------------------------------------------
\subsection{Attention Module Architecture}\label{method:attention}

%\red{[KJ: I am here]}

The goal of \WithinAttention is to update the representations of nodes (or hyperedges) reflecting the \emph{within}-hyperedge relationships between nodes (or hyperedges). %hyperedges (or nodes).
We first introduce \WithinAttention for updating hyperedge embeddings from node embeddings, and then describe the difference in the opposite direction, i.e., updating node embeddings from hyperedge embeddings.
We also employ \PE in both directions of updates, which uses relative node centrality as positional encodings in multi-head attention.

% Our goal is to obtain node representations by reflecting relationships with other nodes within hyperedges.
% We introduce \WithinAttention, which updates the feature of each node as a weighted sum of the embeddings of other nodes within each hyperedge.
% Moreover, we utilize the node centrality as a positional encoding for the attention module.
% Thus, both node centrality and embeddings are considered in measuring pairwise similarities in our attention module.

% where the weight is computed in consideration of the relative node centrality values. \WithinAttention is composed of \WithinAttention and \RankAttention. 
% Here, a node feature $v_i$ maps to \WithinAttention$(\{v_j \forall v_j \in e\}) = $ \WithinAttention(\RankAttention($\{v_j \forall v_j \in e\}$)).

% ------------------------------------------------------------------------
\smallsection{Attention to Interactions within Hyperedges}\label{method:attention:within} 
The attention \linebreak mechanism in \WithinAttention is based on Transformer~\cite{vaswani2017attention}, which updates a set of given embeddings by using itself as queries, keys, and values of attention.
It utilizes edge-dependent relationships between pairs of nodes by calculating dot-product between node pairs within the hyperedge.
% the pairwise interactions between embeddings by calculating the attention weight by the dot-product between two embeddings.
% When queries, keys, and values come from the same embeddings, Transformer updates each feature by a weighted sum of the input embeddings.
% The weight is calculated by the dot-product between two embeddings so that pairwise interactions are considered.
% Thus we can achieve our goal by Transformer taken incident node embeddings as input for queries, keys and values.
However, the computational complexity of considering every node pair is quadratic with the size of each hyperedge, which makes it difficult to be used in large real-world hypergraphs.
Thus, we adopt the strategy proposed in Set Transformer~\cite{lee2019set}. Refer to Section~\ref{attwinducing} for detailed descriptions of the techniques above.

% where queries, keys, and values come from the same node embeddings. Thus each node feature is updated by a weighted sum of the node embeddings within each hyperedge. Here, the weights are calculated by the dot-product between two node embeddings within the hyperedge. 
% Even though it can utilize the pairwise interactions among nodes within each hyperedge, it requires quadratic order of the size of each hyperedge so that it leads to high computations. Thus, we adopt the strategy proposed in Set Transformer~\cite{lee2019set}, as explained in Section~\ref{attwinducing}.

Let $\mathbf{V}_{e}^{(l)} = \{ \mathbf{X}_u^{(l)} : u \in e \}$ denote the set of the embeddings of nodes in a hyperedge $e$ in the $l$-th layer, which are packed into a matrix in $\mathbb{R}^{ |e| \times d_l}$. % in the implementation. 
Along with $\mathbf{V}_{e}^{(l)}$, \WithinAttention uses $m$ number of $d_l$-dimensional trainable inducing points $\mathbf{I}_w \in \mathbb{R}^{m \times d_l}$, where $m$ is typically much smaller than $\max_{e \in \SE} |e|$. In our experiments, $m$ is fixed to $4$.
Then, \WithinAttention is formally expressed as follows:
\begin{equation}
    \WithinAttention(\mathbf{V}_{e}^{(l)} ; \mathbf{I}_w ) = \MultiheadAtt(\mathbf{V}_{e}^{(l)}, \MultiheadAtt(\mathbf{I}_w, \mathbf{V}_{e}^{(l)})).
\end{equation}
Note that $\mathbf{I}_w$ is used globally for all hyperedges.
The inner \MultiheadAtt (defined in Section~\ref{attwinducing}) summarizes the node embeddings in $e$ with a help of $\mathbf{I}_w$.
After that, the outer \MultiheadAtt generates edge-dependent representations of each of $|e|$ nodes based on the relationship between input node embeddings and the summary of them, created by the inner \MultiheadAtt.
As a result, the resulting representations can be interpreted as an approximation of all-pair attention.

% not defined depending on the hyperedge $e$ so that it is 
%so that looking at the relationship between nodes and this summarization could approximate the node-pairwise relationship in $e$ at the second \MultiheadAtt.
%We intend that the information from nodes in $e$ is summarized with the help of $I_w$ and then it is reflected on newly representation of them.

% ------------------------------------------------------------------------
%\smallsection{\RankAttention}\label{method:attention:rank}
\smallsection{Using Centrality for Positional Encoding}\label{method:attention:rank}
Furthermore, to make the edge-dependent relationships between nodes within each hyperedge more explicit, we use the relative order of node centrality within the hyperedge as positional encodings for the attention module, which is named \PE. We define the \textit{order} of each element $a$ in a set $A$ as follows:
\begin{equation}\label{equation:order}
    Order(a, A) = \sum_{a' \in A} \mathds{1}(a' < a)
\end{equation}
Then, for given node centralities $\mathbf{F} \in \mathbb{R}^{N \times d_f}$ where $d_f$ is the number of different types of centralities, which also corresponds to the dimensionality of positional encodings, we define \PE of a node $v$ within a hyperedge $e$ as follows: 
\begin{equation}\label{equation:rank}
    \PE(v, e ; \mathbf{F}) = \parallel_{i=1}^{d_f} \frac{1}{|e|} Order(\mathbf{F}_{v,i}, \{ \mathbf{F}_{u,i} | \forall u \in e \})
\end{equation}
Here, $\parallel$ indicates the concatenation of the order with respect to the centrality of type $i$ for each $1\leq i \leq d_{f}$. We simply add \PE to the node embeddings and feed them into \WithinAttention. In our experiments, we leverage four types of node centrality: degree, eigenvector centrality, PageRank, and coreness. Details of them are described in Appendix ~\ref{appendix:nodecentral}.

% We rank the nodes within each hyperedge $e$ according to centralities and concatenate the rankings.
% \begin{equation}\label{equation:rank}
%     \PE(e;F) =\{ ||_{i=1}^{d_f} \frac{1}{|e|} \sum_{u \in e} \mathds{1}(F_{u,i} < F_{v,i}) : v \in e \}
% \end{equation}
Similarly, for the message passing from hyperedges to nodes, we explicitly give the target node's order within the source hyperedge.
In other words, the same position encoding is used for each hyperedge and node pair in both directions of message passing.
% we input explicit information about the order of the target node centrality within its incident hyperedge. In other words, for hyperedge and node pairs, the same positional encodings are used in both directions of message passing.

% \begin{equation}\label{equation:rank_v}
%     \PE(\mathcal{N}_v;F) = \{ ||_{i=1}^{d_f} \frac{1}{|e|} \sum_{u \in e} \mathds{1}(F_{u,i} < F_{v,i}) : e \in \mathcal{N}_v \}
%     %\{ R_{e,v} : e \in \mathcal{N}_v \}
% \end{equation}
% To simplify, for hyperedge and node pairs, they have same positional encodings in both directions of message passings.  
% We also add \PE to the hyperedge embeddings as the input for \WithinAttention in incident hyperedges.
% By providing explicit information about the relative importance of nodes within hyperedges in the input, we expect the attention mechanism can grasp the node importance signal in addition to the similarity in embeddings, which can be observed in Graphormer~\cite{ying2021transformers}.

% Previous ------------------------------------------------------------
% We design another attention block, \RankAttention, where queries come from node rankings and keys and values come from node embeddings in the neighborhood of a target hyperedge. 
% % which input the above node rankings depending on hyperedges. 
% Along with node embeddings $V_{e} \in \mathbb{R}^{|e| \times d^{(l)}}$ and rankings $R_{e} \in \mathbb{R}^{|e| \times d_f}$, \RankAttention also uses $m$ trainable inducing points $I_r \in \mathbb{R}^{m \times d^{(l)}}$. Since this block also intends to consider node-pairwise relationship, the inducing points are used to avoid the computation of $|e|^{2}$.
% \begin{equation}
%     \RankAttention(V_{e}^{(l)}, R_{e} ; I_r) = \MultiheadAtt(R_{e}, \MultiheadAtt(I_r, V_{e}^{(l)}) 
% \end{equation}
% As $I_w$ in \WithinAttention, $I_r$ is used commonly regardless of hyperedge $e$. This is similar to \WithinAttention, but here we expect both the ranking and the embedding to be considered in assigning weights for the node-pairs in $e$.
%We expect that $H_r$ is small but has enough information about current node embeddings so that it helps express node rankings fluently.

% ------------------------------------------------------------------------
\subsection{Aggregation Module Architecture}\label{method:aggregation}
% Note that, layer 1 == average
%With node embeddings that consider the relationships between neighbor nodes included in the same hyperedge, that is $Z_{e_j} =$ \WithinAttention(\RankAttention($V_{e_j}, R_{e_j}$)), we update each hyperedge's feature by aggregating embeddings of all nodes within it. 
After edge-dependent node embeddings are obtained by \WithinAttention, the hyperedge embedding is computed by aggregating them, through \aggregation.
We aggregate edge-dependent node embeddings with weights obtained by the dot-product between the node embedding and the previous embedding of the hyperedge as follows:
% applying multihead attention between nodes and previous hyperedge feature. 

\begin{equation}
    \mathbf{H}_e^{(l)} = \aggregation(\tilde{\mathbf{V}}_{e}^{(l)}, \mathbf{H}_e^{(l-1)}) = \MultiheadAtt(\mathbf{H}_e^{(l-1)},\tilde{\mathbf{V}}_{e}^{(l)}),
\end{equation}
where $\tilde{\mathbf{V}}_{e}^{(l)} = \WithinAttention(\mathbf{V}_{e}^{(l-1)})$,
$\mathbf{H}_e \in \mathbb{R}^{(1\times d_{l})}$, and $\tilde{\mathbf{V}}_{e} \in \mathbb{R}^{(|e| \times d_l)}$.

% Here, the dimension of $\mathbf{H}_e$ and $\tilde{\mathbf{V}}_{e}$ is $1 \times d_l$ and $|e| \times d_l$ respectively. 

% We later empirically show that such aggregation performs better than weighing node embeddings by attention with a learnable seed vector which is used in Set Transformer~\cite{lee2019set}. 

%simply dimension-wise averaging or applying weights on each node feature by attention with a learnable seed vector which is used in Set Transformer~\cite{lee2019set}. 

% ------------------------------------------------------------------------
\subsection{All Together: \method}\label{method:overall}

We introduce \method, our hypergraph neural network that combines the afore-described modules.
At each layer, edge-dependent node embeddings are first computed by incorporating edge-dependent  relationships between nodes within each hyperedge via \WithinAttention and \PE. 
Then \aggregation outputs hyperedge embeddings through a  weighted sum of edge-dependent node embeddings. 
Similarly, node embeddings are updated by aggregating node-dependent hyperedge embeddings from \WithinAttention which uses node-dependent relationships between hyperedges incident to the corresponding node.
% Using the modules explained above, we introduce our hypergraph neural network, \method.
%, which outputs embeddings of both nodes and hyperedges. We explain how we predict the labels of nodes depending on a certain hyperedge.
%\method first updates each hyperedge feature by aggregating messages from nodes within it which entails relative positions. Then \method updates each node feature by aggregating messages from neighbor hyperedges in the same way.
Specifically, a hyperedge $e$'s embedding is updated as follows:
\begin{equation}
    \mathbf{V}_{e,\boxplus}^{(l)} = \{ \mathbf{X}_v^{(l-1)} \boxplus \PE(v, e)) : v \in e  \},
\end{equation}
\begin{equation}\label{equation:method_att}
    \tilde{\mathbf{V}}_{e}^{(l)} = \WithinAttention(\mathbf{V}_{e,\boxplus}^{(l)}),
\end{equation}
\begin{equation}
    \mathbf{H}_e^{(l)} = \aggregation(\tilde{\mathbf{V}}_{e}^{(l)}, \mathbf{H}_e^{(l-1)}),
    %\MultiheadAtt(H_e^{(l-1)}, \tilde{V}_{e}^{(l)})
\end{equation}
% \begin{equation*}
%     \text{where } V_{e}^{(l-1)} = \{ X_v^{(l-1)} : v \in e \}
% \end{equation*}
% where  $V_{e}^{(l-1)} = \{ X_v^{(l-1)} : v \in e \}$ and 
where $\boxplus$ denotes adding positional encoding after matching the dimension with that of embeddings by a learnable matrix.
% \begin{equation}\label{equation:att_e}
%     \text{where } \tilde{V}_{e}^{(l)} = \WithinAttention(V_{e}^{(l-1)})
% \end{equation}
% Here, the size of $H_e^{(l)}$ is one and that of $\tilde{V}_e^{(l)}$ is $|e|$. 

Then a node $v$'s embedding is updated as follows:

\begin{equation}
    \mathbf{E}_{v,\boxplus}^{(l)} = \{ \mathbf{H}_e^{(l)} \boxplus \PE(v, e)) : e \in \mathcal{N}_{v}  \},
\end{equation}
\begin{equation}
    \tilde{\mathbf{E}}_{v}^{(l)} = \WithinAttention(\mathbf{E}_{v,\boxplus}^{(l)}),
\end{equation}
\begin{equation}
    \mathbf{X}_v^{(l)} = \aggregation(\tilde{\mathbf{E}}_{v}^{(l)}, \mathbf{X}_v^{(l-1)}).
\end{equation}
% \begin{equation*}
%     \text{where } E_{v}^{(l-1)} = \{ H_e^{(l-1)} : e \in \mathcal{N}_{v} \}
% \end{equation*}
% where  $E_{v}^{(l-1)} = \{ H_e^{(l-1)} : e \in \mathcal{N}_{v} \}$.
% \begin{equation}\label{equation:att_v}
%     \text{where } \tilde{E}_{v}^{(l)} = \WithinAttention(E_{v}^{(l)})
% \end{equation}
% Here, the size of $X_v^{(l)}$ is one and that of $\tilde{E}_v^{(l)}$ and $ E_v^{(l-1)}$ are $|\mathcal{N}_v|$.
We also can stack more than one \WithinAttention layers, before aggregating embeddings, in order to capture higher-order (beyond pairwise) relationships among adjacent nodes (hyperedges).

% Finally, with $X_v^{(L)}$ and $H_e^{(L)}$ after stacking $L$ layers, we predict the label of a node $v$ in a hyperedge $e$ as follows,
% \begin{equation}
%     Label_{(v, e)} = SoftMax(FF([X_v^{(L)} || H_e^{(L)}]))
% \end{equation}
% where FF indicates a fully connected layer. We concatenate one hyperedge embedding and one node embedding and input this into a softmax layer so that we get probabilities of node labels dependng on hyperedges.

% ------------------------------------------------------------------------
\subsection{Complexity Analysis}\label{method:analysis}
% Set Transformer reference?
Since we use relatively a small number of inducing points, \WithinAttention requires $O(|e|)$ time for each hyperedge $e$ and $O(|\mathcal{N}_v|)$ time for each node $v$. \aggregation computes the dot-product between a query of size $1$ and a key of size $|e|$ for each hyperedge $e$ so that it  requires $O(|e|)$ time.
Similarly, it computes the dot-product between a query of size $1$ and a key of size $|\mathcal{N}_v|$ for each node $v$ so that it also requires $O(|\mathcal{N}_v|)$ time.
For updating all hyperedges and nodes, the complexity becomes $O(max_{e \in \SE} |e| + max_{v \in \SV} |\mathcal{N}_v|)$. Thus, for $L$ layers, \method takes $O(L (max_{e \in \SE} |e| + max_{v \in \SV} |\mathcal{N}_v|))$ time.

% ------------------------------------------------------------------------
\subsection{Comparison to Existing Models}\label{method:comp}

To efficiently consider edge-dependent relationships between node pairs within hyperedges, we adopt the encoder part of SetTransformer~\cite{lee2019set} as one of the components of message passing in our model.  
SetTransformer aims to make a proper representation of a set, so it is not a model for hypergraphs. And the aggregation module of \method (i.e., \aggregation) differs from the decoder of SetTransformer, named Pooling by Multihead Attention (PMA). Both aggregate input embeddings by the weighted sum, but PMA uses weights by attention to the global learnable parameter and \aggregation uses attention to the previous embedding of the target. Additionally, we employ \PE in the attention module. 
%In appendix~\ref{appendix:abl_agg}, we observe that our \aggregation performs better than PMA. 

There exists an attempt to use SetTransformer as a component of the message passing in hypergraphs like us. AllSetTransformer~\cite{chien2021you} is designed to integrate SetTransformer into hypergraph neural networks. However, it does not adopt the encoder of SetTransformer, and only the decoder module PMA  is used with a slight change in the number of stacking feed-forward layers in the multi-head attention block. Therefore, AllSetTransformer does not utilize interactions among adjacent nodes or hyperedges and just aggregates incident embeddings like PMA.

% Previous ------------------------------------------------------------------------
% SetTransformer~\cite{lee2019set} is most related to our \method. SetTransformer consists of Set Attention Block (SAB) which encodes each set elements by containing interactions among elements in the set and Pooling by Multihead Attention (PMA) which makes a set embedding by aggregating element embeddings. Whereas the SAB has the same structure with our \WithinAttention, SetTransformer is not a hypergraph neural network but is a model that takes a set of instances as an input and makes a proper representation of the set.  Also, it does not use positional encoding in the attention mechanism and our \aggregation is different from PMA. Both aggregations make the influence of each embeddings on the target differently. But we determine the influence by the relationship with the previous target embeddings but PMA considers the relationship with the global learnable vector. In appendix~\ref{}, we observe that our \aggregation performs better than the variant of \method which replaces the \aggregation with PMA.

% Furthermore, AllSetTransformer~\cite{chien2021you} is actually designed to integrate SetTransformer into hypergraph neural networks. However, it does not incorporate SAB and uses only PMA. Therefore, AllSetTransformer does not utilize interactions among incident nodes or hyperedges and just aggregate incident embeddings likewise PMA.

% The \textit{Set Attention Blocks(SAB)} of SetTransformer also consider pairwise interactions among set instances. However, it does not use positional encoding in attention and the aggregation scheme of SetTransformer differs from ours. Additionally, we can also observe that our \Aggregation performs better than the variant of \method which replaces the \aggregation with the aggregation scheme of SetTransformer, \textit{Pooling by Multihead Attention(PMA)}, in Appendix~\ref{}. 

% AllSetTransformer is proposed to integrate SetTransformer into hypergraph neural networks. However, it does not incorporate Set Attention Block. Therefore, AllSetTransformer does not utilize pairwise interactions among nodes or hyperedges.



==> backup/070evaluation.tex <==
% EVALUATION ====================================================================================================================
\begin{table*}[t]
    \vspace{-1mm}
    \begin{center}
        \caption{\label{tab:expresult} \underline{\smash{Results of Edge-Dependent Node Classification}}: Mean and standard deviation of Micro-F1 and Macro-F1 scores over $3$ independent runs are reported. Best scores are in \textbf{bold}. Note that \method performs best in all datasets. HCHA runs out of memory on the coauthorship-AMiner dataset.}
        \scalebox{0.757}{
            \begin{tabular}{l l | c c | c c c c c | c c || c}
            \toprule
            % \multicolumn{2}{c|}{DataSet}
            Dataset & Metric & BaselineU & BaselineP & HNHN & HGNN & HCHA & HAT & UniGCNII & HST & AST & \method\\ 
            \midrule
            \multirow{2}{*}{\shortstack[l]{Coauth-\\DBLP}} & MicroF1 & 0.333 $\pm$ 0.001 & 0.346 $\pm$ 0.001 & 0.490 $\pm$ 0.001 & 0.542 $\pm$ 0.001 & 0.454 $\pm$ 0.007 & 0.505 $\pm$ 0.002 & 0.497 $\pm$ 0.004 & 0.563 $\pm$ 0.000 & 0.526 $\pm$ 0.003 & \textbf{0.605} $\pm$ 0.002 \\
            & MacroF1 & 0.330 $\pm$ 0.001 & 0.332 $\pm$ 0.001 & 0.484 $\pm$ 0.001 & 0.519 $\pm$ 0.003 & 0.360 $\pm$ 0.045 & 0.486 $\pm$ 0.006 & 0.476 $\pm$ 0.003 & 0.547 $\pm$ 0.000 & 0.520 $\pm$ 0.003 & \textbf{0.594} $\pm$ 0.003\\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Coauth-\\AMiner}} & MicroF1 & 0.334 $\pm$ 0.000 & 0.339 $\pm$ 0.000 & 0.521 $\pm$ 0.002 & 0.566 $\pm$ 0.003 & OutOfMemory & 0.541 $\pm$ 0.001 & 0.521 $\pm$ 0.000 & 0.595 $\pm$ 0.008 & 0.581 $\pm$ 0.000 & \textbf{0.627} $\pm$ 0.004\\
            & MacroF1 & 0.332 $\pm$ 0.000 & 0.333 $\pm$ 0.000 & 0.515 $\pm$ 0.002 & 0.553 $\pm$ 0.001 & OutOfMemory & 0.531 $\pm$ 0.003 & 0.507 $\pm$ 0.001 & 0.584 $\pm$ 0.004 & 0.572 $\pm$ 0.001 & \textbf{0.621} $\pm$ 0.006\\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Email-\\Enron}} & MicroF1 & 0.334 $\pm$ 0.001 & 0.439 $\pm$ 0.001 & 0.733 $\pm$ 0.029 & 0.723 $\pm$ 0.005 & 0.668 $\pm$ 0.005 & 0.817 $\pm$ 0.001 & 0.741 $\pm$ 0.003 & 0.818 $\pm$ 0.003 & 0.807 $\pm$ 0.001 & \textbf{0.826} $\pm$ 0.001\\
            & MacroF1 & 0.300 $\pm$ 0.001 & 0.333 $\pm$ 0.001 & 0.633 $\pm$ 0.022 & 0.673 $\pm$ 0.003 & 0.465 $\pm$ 0.001 & 0.755 $\pm$ 0.003 & 0.658 $\pm$ 0.012 & 0.752 $\pm$ 0.008 & 0.735 $\pm$ 0.001 & \textbf{0.760} $\pm$ 0.003\\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Email-\\Eu}} & MicroF1 & 0.500 $\pm$ 0.001 & 0.525 $\pm$ 0.001 & 0.642 $\pm$ 0.004 & 0.633 $\pm$ 0.001 & 0.621 $\pm$ 0.000 & 0.669 $\pm$ 0.001 & 0.633 $\pm$ 0.002 & \textbf{0.671} $\pm$ 0.001 & 0.669 $\pm$ 0.001 & \textbf{0.671} $\pm$ 0.000\\
            & MacroF1 & 0.493 $\pm$ 0.001 & 0.499 $\pm$ 0.001 & 0.548 $\pm$ 0.015 & 0.530 $\pm$ 0.008 & 0.497 $\pm$ 0.001 & 0.640 $\pm$ 0.003 & 0.560 $\pm$ 0.012 & 0.639 $\pm$ 0.001 & 0.639 $\pm$ 0.001 & \textbf{0.644} $\pm$ 0.002\\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Stack- \\Biology}} & MicroF1 & 0.335 $\pm$ 0.000 & 0.368 $\pm$ 0.001 & 0.636 $\pm$ 0.006 & 0.690 $\pm$ 0.001 & 0.587 $\pm$ 0.002 & 0.659 $\pm$ 0.006 & 0.605 $\pm$ 0.004 & 0.698 $\pm$ 0.003 & 0.718 $\pm$ 0.002 & \textbf{0.738} $\pm$ 0.001\\
            & MacroF1 & 0.326 $\pm$ 0.000 & 0.334 $\pm$ 0.003 & 0.585 $\pm$ 0.001 & 0.626 $\pm$ 0.006 & 0.417 $\pm$ 0.003 & 0.604 $\pm$ 0.008 & 0.425 $\pm$ 0.004 & 0.638 $\pm$ 0.001 & 0.645 $\pm$ 0.003 & \textbf{0.680} $\pm$ 0.003\\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Stack- \\Physics  }} & MicroF1 & 0.333 $\pm$ 0.001 & 0.370 $\pm$ 0.000 & 0.548 $\pm$ 0.016 & 0.688 $\pm$ 0.005 & 0.622 $\pm$ 0.004 & 0.709 $\pm$ 0.004 & 0.664 $\pm$ 0.026 & 0.756 $\pm$ 0.013 & 0.759 $\pm$ 0.003 & \textbf{0.773} $\pm$ 0.002\\
            & MacroF1 & 0.322 $\pm$ 0.001 & 0.332 $\pm$ 0.000 & 0.447 $\pm$ 0.038 & 0.631 $\pm$ 0.003 & 0.481 $\pm$ 0.008 & 0.642 $\pm$ 0.009 & 0.487 $\pm$ 0.019 & 0.660 $\pm$ 0.013 & 0.680 $\pm$ 0.006 & \textbf{0.707} $\pm$ 0.002\\
            \bottomrule
        \end{tabular}}
    \end{center}
\end{table*}
% ====================================================================================================================
\begin{table*}[t]
    \vspace{-2mm}
    \begin{center}
        \caption{\label{tab:jsdresult} \underline{\smash{Jensen-Shannon divergence (JSD) between Ground-truth and Predicted Node Label Distributions}}: The average and standard deviation of the average JSD over $3$ independent runs are reported.
        The lower JSD is, the better a model preserves node-level label distributions.
        Best scores are in \textbf{bold}.
        \method yields the lowest JSD in almost all datasets.}
        \scalebox{0.77}{
            \begin{tabular}{l| c c | c c c c c | c c || c}
            \toprule
            % \multicolumn{2}{c|}{DataSet}
            Dataset & BaselineU & BaselineP & HNHN & HGNN & HCHA & HAT & UniGCNII & HST & AST & \method\\
            \midrule
            Coauth-DBLP & 0.532 $\pm$ 0.002 &  0.518 $\pm$ 0.002 &  0.449 $\pm$ 0.001 &  0.391 $\pm$ 0.002 &  0.451 $\pm$ 0.002 &  0.427 $\pm$ 0.003 &  0.450 $\pm$ 0.007 &  0.387 $\pm$ 0.000 &  0.423 $\pm$ 0.001 &  \textbf{0.349} $\pm$ 0.002 \\ 
            Coauth-AMiner & 0.529 $\pm$ 0.000 &  0.523 $\pm$ 0.000 &  0.438 $\pm$ 0.003 &  0.372 $\pm$ 0.003 & OutOfMemory &  0.413 $\pm$ 0.003 &  0.423 $\pm$ 0.000 &  0.357 $\pm$ 0.006 &  0.375 $\pm$ 0.001 &  \textbf{0.330} $\pm$ 0.003 \\ 
            Email-Enron & 0.486 $\pm$ 0.002 &  0.395 $\pm$ 0.001 &  0.164 $\pm$ 0.001 &  0.214 $\pm$ 0.008 &  0.290 $\pm$ 0.008 &  0.156 $\pm$ 0.002 &  0.188 $\pm$ 0.002 &  0.154 $\pm$ 0.003 &  0.162 $\pm$ 0.002 &  \textbf{0.136} $\pm$ 0.001 \\ 
            Email-Eu & 0.199 $\pm$ 0.006 &  0.164 $\pm$ 0.004 &  0.234 $\pm$ 0.011 &  0.291 $\pm$ 0.001 &  0.268 $\pm$ 0.002 &  \textbf{0.152} $\pm$ 0.003 &  0.297 $\pm$ 0.001 &  0.160 $\pm$ 0.003 &  0.157 $\pm$ 0.006 &  0.155 $\pm$ 0.009 \\ 
            Stack-Biology & 0.536 $\pm$ 0.001 &  0.467 $\pm$ 0.003 &  0.273 $\pm$ 0.008 &  0.202 $\pm$ 0.004 &  0.221 $\pm$ 0.002 &  0.237 $\pm$ 0.006 &  0.261 $\pm$ 0.002 &  0.197 $\pm$ 0.007 &  0.186 $\pm$ 0.003 &  \textbf{0.155} $\pm$ 0.001 \\ 
            Stack-Physics & 0.532 $\pm$ 0.001 &  0.482 $\pm$ 0.001 &  0.262 $\pm$ 0.016 &  0.215 $\pm$ 0.008 &  0.288 $\pm$ 0.005 &  0.230 $\pm$ 0.004 &  0.298 $\pm$ 0.059 &  0.160 $\pm$ 0.009 &  0.168 $\pm$ 0.002 &  \textbf{0.140} $\pm$ 0.002 \\ 
            \bottomrule
        \end{tabular}}
    \end{center}
\end{table*}
% ====================================================================================================================

We evaluate \method by answering the following questions:

\begin{itemize}[leftmargin=*]
    \item \textbf{Q1.} Does \method accurately predict the edge-dependent labels of nodes?
    \item \textbf{Q2.} Does \method classify the same node  differently depending on hyperedges? %Isn't the high performance of classification obtained by predicting the most frequent labels for nodes?
    \item \textbf{Q3.} Does each component of \method make a meaningful contribution to the performance?
    \item \textbf{Q4.} How can we apply \method to a real-world downstream task? Does \method outperform baseline approaches?
\end{itemize}

% ====================================================================================================================
% \subsection{Datasets}
% We used $6$ datasets from $3$ domains described in Section~\ref{benchmarkdataset}. 
% The properties of datasets are summarized in Table~\ref{tab:datasets}. 

% \noindent \textbf{Co-authorship} (DBLP and AMinerAuthor) : Each hyperedge represents a publication consisting of co-authors. The node labels are assigned by first, last, and other authors in each publication.

% \noindent \textbf{Email} (Enron and Eu): Each hyperedge represents an email and the nodes in it are separated by sender, receiver, and cc (carbon copy).

% \noindent \textbf{StackOverflow} (Biology and Physics): Each hyperedge represents a post, and nodes are divided into the questioner, the answerer adopted by the questioner, and the other answerers of the post.

% Additionally, we analyze the correlation between relative node centralities and hyperedge-dependent node labels in each dataset. In detail, we calculate Cramer's coefficient matrix[] between $R_e$ defined in ~\ref{equation:rank} and labels of nodes in $e$ over all hyperedges. We report the correlation value according to each node centrality, i.e. degree, eigenvector, pagerank and k-coreness,  and average in Table~\ref{tab:datasets}.

% ====================================================================================================================
%\subsection{Comparative Models}

%We even extend the ablation study in a relatively small dataset, StackOverflow-Biology. The result is described in Appendix~\ref{}.
%They are designed to support our model in Section~\ref{sec:ablation}.

% ====================================================================================================================
\subsection{Experimental settings}
\label{sec:exp:setting}
\smallsection{Competitors}
As competitors, we use $6$ hypergraph neural networks that generate both hyperedge and node embeddings and thus can be used for edge-dependent node classification: HNHN~\cite{dong2020hnhn}, HGNN~\cite{feng2019hypergraph}, HCHA~\cite{bai2021hypergraph}, HAT~\cite{hwang2021hyfer}, UniGCNII~\cite{huang2021unignn}, and AllSetTransformer (AST) ~\cite{chien2021you}.
We implemented them all using Deep Graph Library (DGL) ~\cite{wang2019deep}. 
We exclude HyperGCN~\cite{yadati2019hypergcn} from the competitors since it does not provide hyperedge embeddings. %replaces hyperedges with representative pair edges and thus the information about hyperedges is removed after replacement.
%also tries to apply convolution in hypergraph like HGNN. But it does not compute hyperedge embeddings directly because hyperedges are replaced by the connections to two mediator nodes. 
%We experimented not only HCHA, which learns the attention between the hyperedge and the node, but also HAT~\cite{hwang2021hyfer}, which applies attention to aggregation at hyperedges and aggregation at nodes separately. 
SetTransformer~\cite{lee2019set} is closely related to our work, and used as a component of \method, but cannot be applied directly to our problem.
% SetTransformer~\cite{lee2019set} is highly related to our model but designed for set embeddings.
Thus, we extend SetTransformer to hypergraphs by applying it to obtain the representations of sets of incident nodes and hyperedges in the two stages of message passing, and we call it HypergraphSetTransformer (HST). 
% The details of competitors are described in Appendix~\ref{appendix:baseline}. 
In addition, we add two simple approaches for comparison: (a) \textit{BaselineU}, which predicts node labels uniformly at random and (b) \textit{BaselineP}, which randomly assign labels proportionally to their global distribution. 
%  to show the non-triviality of our new benchmark problem

% We trained models in mini-batch settings and sampled hyperedges during the node update phase due to memory and time complexity. Exceptionally, HCHA is trained in full-batch settings and we don't use sampling during training.
%, and the hyperedges were updated through all included nodes without sampling.
\smallsection{Other Settings}
%\red{Please refer to a section for datasets}
We use the $6$ real-world datasets described in Section~\ref{benchmark_dataset}.
Since the datasets do not contain node features, we generate initial node features based on the 2nd-order random walks on hypergraphs using Node2Vec \cite{grover2016node2vec}, as described in HyperSAGNN~\cite{zhang2019hyper}.
With the same parameter setting as HyperSAGNN, we construct a fixed-length random walk of each node and obtain embeddings using a skip-gram model~\cite{mikolov2013efficient,mikolov2013distributed}.
%Since they do not contain external node features, we use the 128 dimensional embeddings obtained by .
We randomly divide all hyperedges in each hypergraph into training (60\%), validation (20\%), and test (20\%) sets.
%When we use rankings, we consider 4 node centrality values: degree, eigenvector, pagerank, and k-coreness centralities. => in the method part & appendix 
For all experiments, we train embedding models using a single-layer MLP as the classifier. We use the Adam optimizer and stop training when the number of epochs reaches $100$ or the accuracy on the validation set no longer improves during $25$ epochs. We use the search space described in Appendix~\ref{appendix:hp} for hyperparameter tuning. For each model and each dataset, we choose a setting where the mean of Micro-F1 and Macro-F1 scores on the validation set is maximized and report its performance on the test set over three independent runs. 

\begin{figure}[t]
    \begin{minipage}{0.74\linewidth}
        \includegraphics[width=1.03\linewidth]{FIG/result/embedding_ex2.jpg}
        % \subcaption{Embeddings of publications containing "Hans-Peter Kriegel"}
    \end{minipage}
    \begin{minipage}{0.25\linewidth}
        \includegraphics[width=1.0\linewidth]{FIG/result/embedding_ex4.jpg}
        % \subcaption{Concatenated Embeddings of hyperedges and nodes}
    \end{minipage}
    
    \begin{minipage}{0.56\linewidth} \small
        (a) Embeddings of publications containing "Hans-Peter Kriegel"
    \end{minipage}
    \quad
    \quad
    \begin{minipage}{0.32\linewidth} \small
        (b) Concatenated Embeddings of hyperedges and nodes
    \end{minipage}
    
    \caption{\underline{\smash{Visualization of embeddings from \method}}: (a) As an example of discernable label-specific clustering of hyperedge embeddings, the embeddings of all publications of ``Hans-Peter Kriegel'' are visualized using LDA. (b) The concatenated embedding of hyperedge and node pairs in the test dataset are visualized using LDA, where colors represent edge-dependent node labels.}
\end{figure}

% ====================================================================================================================
\subsection{Q1. Edge-Dependent Node Classification}

In order to evaluate \method in edge-dependent node classification, we measure the predictive performances of all the considered models in terms of Micro-F1 and Macro-F1 scores on the test data averaged over three runs.
As shown in Table~\ref{tab:expresult}, \method consistently outperforms all the competitors in terms of both Micro-F1 and Macro-F1. 
HST and AST are usually second best.
As described in detail in Section~\ref{method:comp}, HST, AST, and \method  use different aggregation methods. Moreover, the relationships among adjacent nodes and hyperedges are considered only in HST and \method, and the positional encoding is only used in \method. The fact that AST underperforms HST and \method supports the effectiveness of \WithinAttention. Furthermore, the fact that \method outperforms HST supports the usefulness of the \aggregation module and \PE.
While HGNN performs particularly well on the Coauth-DBLP dataset and HAT performs well on the Email-Enron and Eu datasets, their overall performance was not good.
HCHA runs out of memory on the Coauth-AMiner dataset, and its performance is poor in the other datasets.
% As a result of searching the proper number of stacks of \WithinAttention, two stacks of \WithinAttention perform better than one single stack in most datasets (See Appendix~\ref{}). This implies that higher-order more than pairwise interactions is constitutive.
% [Temporary: compared to HST -> show benefit of our PE and aggregation module ; AST -> attention]
% And AST has high performance compared to other competitors, but it is outperformed by our \method in all datasets.
% As SetTransformer performs poorly especially on Coauthorship-DBLP and Email-Enron where it even showed lower performance than a model that does not learn weights for each node, we assume that it may not be suitable for learning on hypergraph. 
% [HAT & HST & AST]
% Furthermore, the fact that HAT achieves high performance well on average after our \method and AllSetTransformer implies the importance of weighting differently for nodes in our problem. 

% ====================================================================================================================
\subsection{Q2. Node Label Distribution Preservation}\label{sec:evaluation:labeldist}

% What's special about our benchmark is the situation where the labels of nodes vary depending on the hyperedge. (As you can check in Table~\ref{tab:datasets}, the actual dataset has a nonzero average of the entropy in the label distribution of each node.) We wanted to see if the model grasped this by making similar distribution of node labels depending on the hyperedges as the answer. Thus, we measure the Jensen-Shannon divergence between distributions of labels of each node in incident hyperedges from the prediction and the answer, and then average them over all nodes. 
% Table ~\ref{tab:jsdresult} reports the mean and standard deviation of the average Jensen-Shannon divergence in independent $3$ runs on the test dataset. \method has the lowest divergence in most datasets except for Email-Eu, which means that it preserves the distribution of labels of each node well. Even in Email-Eu, it showed the lowest after HAT.

In edge-dependent node-label classification, a single node can have different labels for different hyperedges. That is, each node $v \in \SV$ has its own ground-truth label distribution (node-level label distribution), which describes how many times it has each label. 
In this experiment, we aim to check how well \method preserves such node-level label distributions compared to other baseline approaches.
To this end, we measure the Jensen-Shannon divergence (JSD) \cite{lin1991divergence} between the ground-truth node-level label distribution and the predicted node-level label distribution for every node $v \in \SV$ in the test data.
The average of JSD values for all nodes is regarded as a metric that measures how well a model captures the ground-truth node-level label distribution.
We report the mean and standard deviation of the average JSD over three independent runs in Table~\ref{tab:jsdresult}.
\method shows the lowest JSD in most datasets except for Email-Eu, and it is second-best even in Email-Eu.
This result means that \method effectively preserves the ground-truth node-level label distribution.

% Then, we get an average of every node's JSD value, and regard this computed average as a metric that explains how well a specific model captures the ground-truth node-level label distribution on a specific dataset.
% For each model-dataset pair, we obtain the mentioned metric on three different data splits, and report the average as a final score.
% We measure the Jensen-Shannon divergence between label distributions of each node from the prediction and the answer and average over nodes in test dataset. We report the average Jensen-Shannon divergence in the experiment of $3$ runs in Table~\ref{tab:jsdresult}. Except Email-Eu, our \method makes the most similar distribution of labels of a node for hyperedges. In Email-Eu, \method wo. \WithinAttention performs better but the gap is quite small as $0.001$.

% ====================================================================================================================
% \begin{figure}[t]
%     \includegraphics[width=1.0\linewidth]{FIG/result/embedding_ex3.jpg}
%     \caption{Result of \method embedding }
% \end{figure}


% ====================================================================================================================

% ====================================================================================================================
\begin{table*}[t]
    \vspace{-2mm}
    \caption{\label{tab:downstream}\underline{\smash{Real-World Applications of \method:}} In the three real-life applications, utilizing hypergraphs with edge-dependent node labels predicted by \method shows better performance than using hypergraphs without such labels. The results support the usefulness of identifying edge-dependent node labels by \method in various applications.}
    % \vspace{-0.3cm}
    \begin{subtable}{.3\linewidth}
        \centering
        \caption{Ranking Aggregation}
        \scalebox{0.8}{
    	\begin{tabular}{l|c}
    		\toprule
    		Method & Accuracy \\ 
    		\midrule
    		TrueSkill & \textbf{73.4} \% \\
    		\textbf{Hypergraph w/ \method} & \underline{71.8} \% \\
    		Hypergraph w/ GroundTruth & 71.1 \% \\
    		Clique Graph & 61.1 \% \\
    		Hypergraph w/o Labels & 53.2 \% \\
    		MC3 & 52.9 \% \\
    		\bottomrule
        \end{tabular}}
    \end{subtable}% 
	\hspace{0.5cm}
    \begin{subtable}{.3\linewidth}
        \centering
        \caption{Clustering (NMI: The higher, the better)}
        \scalebox{0.8}{
        \begin{tabular}{l|c}
			\toprule
			Method & NMI Score\\
			\midrule
			Hypergraph w/ GroundTruth & \textbf{0.2209} \\
			\textbf{Hypergraph w/ \method} & \underline{0.2146} \\
			Hypergraph w/o Labels & 0.1634 \\
			\bottomrule
		\end{tabular}}
	\end{subtable}
	\hspace{0.5cm}
	\begin{subtable}{.3\linewidth}
	    \centering
	    \caption{Product Return Prediction}
        \scalebox{0.8}{
        \begin{tabular}{l|c}
        	\toprule
        	Method & Precision\\
        	\midrule
        	HyperGO w/ GroundTruth & \textbf{0.7553}\\
        	\textbf{HyperGO w/ \method} & \underline{0.7536} \\
        	HyperGO w/o Labels &  0.7526 \\ 
        	\bottomrule
        \end{tabular}}
    \end{subtable}
\end{table*}

% ====================================================================================================================
\begin{table}[t]
    \begin{center}
        \caption{\label{tab:ablresult} \underline{\smash{Ablation Study of \method:}} The performance of \method is largely improved by \WithinAttention and \PE, as shown in the average rankings of models.}
        % The average rankings of three models in Micro / Macro-F1 score over datasets show the large improvement by \WithinAttention and the effectiveness of using \PE.}
        \scalebox{0.8}{
            \begin{tabular}{l l| c c c}
            \toprule
            % \multicolumn{2}{c|}{DataSet} 
            Dataset & Metric & w/o \WithinAttention & w/o \PE & \method\\
            %\cmidrule{3-4} \cmidrule{6-7} \cmidrule{11-12} \cmidrule{14-15} \\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Coauth-\\DBLP}} & MicroF1 & 0.583 $\pm$ 0.004 & 0.589 $\pm$ 0.003 & \textbf{0.605} $\pm$ 0.002 \\
             & MacroF1 & 0.579 $\pm$ 0.003 & 0.582 $\pm$ 0.003 & \textbf{0.594} $\pm$ 0.003 \\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Coauth-\\AMiner}} & MicroF1 & 0.612 $\pm$ 0.001 & \textbf{0.629} $\pm$ 0.002 & 0.627 $\pm$ 0.004 \\
             & MacroF1 & 0.602 $\pm$ 0.001 & \textbf{0.622} $\pm$ 0.002 & 0.621 $\pm$ 0.006 \\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Email-\\Enron}} & MicroF1 & 0.819 $\pm$ 0.002 & 0.825 $\pm$ 0.000 & \textbf{0.826} $\pm$ 0.001 \\
             & MacroF1 & 0.758 $\pm$ 0.006 & \textbf{0.762} $\pm$ 0.004 & 0.760 $\pm$ 0.003 \\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Email-\\Eu}} & MicroF1 & 0.665 $\pm$ 0.003 & 0.670 $\pm$ 0.000 & \textbf{0.671} $\pm$ 0.000 \\
             & MacroF1 & 0.641 $\pm$ 0.005 & 0.638 $\pm$ 0.003 & \textbf{0.644} $\pm$ 0.002 \\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Stack-\\Biology}} & MicroF1 & 0.727 $\pm$ 0.000 & 0.734 $\pm$ 0.004 & \textbf{0.738} $\pm$ 0.001 \\
             & MacroF1 & 0.647 $\pm$ 0.010 & \textbf{0.680} $\pm$ 0.002 & \textbf{0.680} $\pm$ 0.003 \\
            \midrule
            \multirow{2}{*}{\shortstack[l]{Stack-\\Physics}} & MicroF1 & 0.756 $\pm$ 0.001 & 0.765 $\pm$ 0.002 & \textbf{0.773} $\pm$ 0.002 \\
             & MacroF1 & 0.671 $\pm$ 0.012 & 0.689 $\pm$ 0.008 & \textbf{0.707} $\pm$ 0.002 \\
            \midrule
            \midrule
            \multirow{2}{*}{\shortstack[l]{AVG.\\Ranking}} & MicroF1 & 3.00 & 1.84 & \textbf{1.17} \\
            & MacroF1 & 2.83 & 1.67 & \textbf{1.33} \\
            \bottomrule
        \end{tabular}}
    \end{center}
\end{table}
% ===================================================================================================================
% \begin{table}[t]
%     \caption{\underline{Downstream Tasks with \method}: On the real-life downstream tasks, utilizing hypergraphs with edge-dependent node labels predicted by \method show better performance than hypergraphs without labels.}
%     % \vspace{-0.3cm}
%     % \begin{center}
%     % \scalebox{0.87}{
%     %     \begin{tabular}{l| c |c}
%     %         \toprule
%     %          & Method & Accuracy \\
%     %         \midrule
%     %         \multirow{6}{*}{\shortstack{Ranking\\Aggregation}} & TrueSkill & \textbf{73.4}\% \\
%     %         & \textbf{Hypergraph w/ \method} & \underline{71.8} \% \\
%     %         & Hypergraph w/ GroundTruth & 71.1 \% \\
%     %         & Clique Graph & 61.1 \% \\
%     %         & Hypergraph w/o Labels & 53.2 \% \\
%     %         & MC3 & 52.9 \% \\
%     %         \midrule
%     %          & Method & NMI Score \\
%     %         \midrule
%     %         \multirow{3}{*}{Clustering} & Hypergraph w/ GroundTruth & \textbf{0.2209} \\
%     %         & \textbf{Hypergraph w/ \method} & \underline{0.2146} \\
%     %         & Hypergraph w/o Labels & 0.1634 \\
%     %         \bottomrule
%     %     \end{tabular}}
%     % \end{center}
%     \begin{subtable}{1.0\linewidth}
%         \centering
%         \caption{Ranking Aggregation}
%         \scalebox{0.86}{
%     	\begin{tabular}{l|c}
%     		\toprule
%     		Method & Accuracy \\ 
%     		\midrule
%     		TrueSkill & \textbf{73.4} \% \\
%     		Hypergraph w/ GroundTruth & 71.1 \% \\
%     		\textbf{Hypergraph w/ \method} & \underline{71.8} \% \\
%     		Clique Graph & 61.1 \% \\
%     		Hypergraph w/o Labels & 53.2 \% \\
%     		MC3 & 52.9 \% \\
%     		\bottomrule
%         \end{tabular}}
%     \end{subtable}% 
% % 	\hspace{0.2cm}

%     \begin{subtable}{1.0\linewidth}
%         \centering
%         \caption{Clustering}
%         \scalebox{0.86}{
%         \begin{tabular}{l|c}
% 			\toprule
% 			Method & NMI Score\\
% 			\midrule
% 			Hypergraph w/ GroundTruth & \textbf{0.2209} \\
% 			\textbf{Hypergraph w/ \method} & \underline{0.2146} \\
% 			Hypergraph w/o Labels & 0.1634 \\
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% \end{table}



% ====================================================================================================================
\subsection{Q3. Ablation Study of \method}
For an ablation study, we compare \method with two variants of it: (a) \textit{\method w/o \WithinAttention}, where \WithinAttention is removed and only \aggregation is used for message passing, and (b) \textit{\method w/o \PE}, which computes \WithinAttention without positional encodings. Table~\ref{tab:ablresult} compares their performances.

\smallsection{Importance of \WithinAttention}
\method consistently outperforms \method w/o \WithinAttention, demonstrating that considering relationships among adjacent nodes and hyperedges is necessary for accurate prediction of edge-dependent node labels, which is consistent with our main motivation. 
The improvement is also contributed by considering the relationships among adjacent hyperedges, as we show this 
in Appendix~\ref{appendix:abl_partial} by testing a variant where \WithinAttention is removed only from the hyperedge to node aggregation step.

\smallsection{Usefulness of \PE}
On average, \method performs better than \method w/o \PE in terms of both Micro F1 and Macro F1 scores. 
Especially in the Coauth-DBLP and Stack-Physics datasets, \method significantly outperforms \method w/o \PE.
We conclude that \PE tends to improve the performance of \method.
In addition, we conduct additional experiments in Appendix~\ref{appendix:abl_pe} to verify the superiority of \PE over other schemes for positional encodings of nodes in  hypergraphs (including global order of node centrality).
% Therefore, the improvement by \PE supports that applying 
% In addition, to compare with other possible positional encodings, we conduct experiments in Appendix~\ref{appendix:abl_pe}.

% =========================================================================================================
\subsection{Q4. Usefulness in Downstream Tasks}
In order to evaluate the usefulness of \method, we consider three applications described in Section~\ref{benchmark_application}. We compare the results using as inputs three different hypergraphs, which are with (a) all ground-truth edge-dependent node labels, (b) those predicted by \method, and (c) no label, respectively. We intend to analyze how useful it is to identify edge-dependent node labels via \method. % compared with the hypergraph without edge-dependent node labels.
How edge-dependent node labels are used for each downstream task is described in Appendix~\ref{appendix:downstream}.

On the Ranking aggregation task, we use a random-walk based method which performed well on this task \cite{chitra2019random}. 
We evaluate the accuracy of predicting the winner in one-to-one matches. We also consider additional competitors used in  \cite{chitra2019random}.
%Using the best clustering method for hypergraph~\cite{hayashi2020hypergraph}, we evaluate whether the publications are grouped well according to their published conferences in the Coauthorship data, which is calculated by NMI score.
On the clustering task, we evaluate whether the publications are grouped well by using venues as their ground-truth cluster. As the backbone hypergraph clustering algorithm, we used a well-performing method~\cite{hayashi2020hypergraph}.
%Finally, the SOTA method, HyperGo~\cite{li2018tail}, is used in the product return prediction task. The performance is measured by precision in predicting the probability of products being returned in the target baskets.
At last, On the product return prediction task, we measured precision of the predicted product return probability of products in the target baskets. We used a SOTA method, HyperGo~\cite{li2018tail}, as the predictor.

% using -> together with
As shown in Table~\ref{tab:downstream}, predicting edge-dependent node labels together with \method led to performance improvement in all applications. Surprisingly, in ranking aggregation, the performance is even higher than knowing the ground-truth. A detailed description of above experiment can be found in Appendix~\ref{appendix:downstream}.
% We also assess the usefulness of our model by applying it in real life. As described in Section~\ref{benchmark_application}, there exist many applications for our model.
% We train our model as an edge-dependent node label predictor while the downstream task is unknown. We then predict all the edge-dependent node labels in the given hypergraph and apply a hypergraph-based algorithm for the downstream task.
% At this time, the algorithm puts different weights on the influence of nodes for each hyperedge, and the predicted edge-dependent node labels can give information on determining these weights.
% We intend to analyze how effective it is to identify edge-dependent node labels via our model compared with the hypergraph without edge-dependent node labels which leads to nodes with uniform weights.

% The advantage of considering nodes differently depending on the hyperedge has been demonstrated in many studies. 
% To show the usefulness of our \method in real-world applications, we also evaluate our \method on the following three downstream tasks. For downstream tasks, we train our model to predict edge-dependent node weights and construct a hypergraph with edge-dependent node weights estimated from our trained model. We aim to analyze the advantage of knowing edge-dependent node weights by comparing the performance of algorithm on the hypergraph with estimated edge-dependent node weights and that on the hypergraph with uniform node weights.

% \smallsection{Ranking Aggregation} % --------------------------------------------------------------------------------------------------------------

% \noindent\textbf{Data.} We experiment with the ranking aggregation with the Halo 2 game dataset as introduced in ~\cite{chitra2019random}. The Halo 2 game dataset consists of two kinds of matches: 31,028 free-for-all matches and 5,093 1-v-1 matches among 5,507 players. The free-for-all matches where up to 8 players play together are used for estimating the overall rankings of players. The 1-v-1 matches where only two players compete are used to evaluate how accurately each method predicts the winner. Players and matches are taken as nodes and hyperedges when modeling data into a hypergraph. And the players can be classified by their contribution level for each match.

% \noindent\textbf{Training.}
% Based on the continuous value of the score gotten by each player in the match, we employ data binning and use the binning index to indicate the contribution level of each player in the match, i.e., edge-dependent node labels. In detail, we normalize the scores for each match and divide the normalized scores into five bins containing 1/5 (20\%) of the total. We train our model with free-for-all matches by splitting them into train/valid/test and predict all edge-dependent node labels in free-for-all matches. On the hypergraphs with predicted edge-dependent node labels, the overall ranking of players is estimated by the stationary distribution of the random walks as following~\cite{chitra2019random}. During the random walks, the node with a higher contribution level is visited more frequently within the hyperedge. In the evaluation of the 1-v-1 matches, we predict the winner as the one with the higher stationary probability. 

% \noindent\textbf{Results.} 
% We compare results with four competitors described in ~\cite{chitra2019random}: ranking aggregation based on random walks on a hypergraph with ground-truth scores and clique graph, a Markov chain-based ranking aggregation ~\cite{dwork2001rank} denoted as MC3, and TrueSkill developed by Microsoft~\cite{herbrich2006trueskill}. Additionally, we analyze the improvement from a hypergraph without edge-dependent node labels which tells just which players played together. 
% The result of applying \method shows the second-highest performance among competitors. Surprisingly, its performance is even higher than that of a hypergraph with a ground-truth score. Hence, we can show that applying binning could lead to better performance. Our performance is quite comparable to TrueSkill, and 8.3\% of 1-v-1 matches are correctly predicted by our model, whereas those missed by TrueSkill. 

% \smallsection{Clustering}\label{sec:eval_downstream_clustering}  % --------------------------------------------------------------------------------------------------------------

% \noindent\textbf{Data.} We experiment with data extracted from Coauthorship-DBLP. We select hyperedges that belong to only one category of computer science, data engineering, software engineering, and theory. Then we choose a set of hyperedges among them, making one connected component. The extracted data consists of 33,050 hyperedges (publications) and 52,560 nodes (authors). In this data, edge-dependent node labels represent the author's position in each publication and are classified into three categories, as described in section~\ref{benchmark_dataset}.
% \textbf{Training.} We train \method to predict the author's position in each publication. After predicting all authors' positions according to publications, we weigh the first or last author by two, and the middle by one as following ~\cite{chitra2019random}. 
% % \begin{equation*}\label{equation:nodeweight_clustering}
% %     \gamma_{e}(v) = \begin{cases}
% %  2 & \text{ if the vertex } v \text{ is the first or last author of publication} \\
% %  1 & \text{ if the vertex } v \text{ is a middle author of publication}
% % \end{cases}
% % \end{equation*}
% Then we apply the clustering algorithm (RDC-Spec) proposed in ~\cite{hayashi2020hypergraph}. Specifically, the stationary distribution of random walks, which proceed in consideration of node weights, is used for spectral clustering.
% \textbf{Results.} We compare the performance of RDC-Spec on three different hypergraphs; ground-truth, predicted, and unknown author positions. The way to weigh according to the author's position is the same as above. In that the result of using \method comes between knowing the ground-truth and not knowing at all, we could assert that capturing the author's position in the publication, i.e., edge-dependent node label is beneficial.

% \smallsection{Product Return Prediction}  % --------------------------------------------------------------------------------------------------------------

% \noindent\textbf{Data.} We use a synthetic dataset from ~\cite{li2018tail} for the product return prediction task. It consists of 6,000 baskets and 10,000 products, which are taken as nodes and hyperedges, respectively. The return rate of each product is assigned by the truncated normal distribution with 0.5 mean and 1.0 standard deviation. The count of products in each basket is determined from 1 to 3 with the probabilities 60\%, 30\%, and 10\%. The baskets are classified by the count of products in them.
% \textbf{Training.} We directly use the count of products in each basket as edge-dependent node labels and train our \method to classify the labels into 1, 2, or 3. We then run HyperGo algorithm~\cite{li2018tail} on the hypergraph with predicted counts.
% \textbf{Results.} Similar to the previous clustering task, we compare the result of HyperGo on three different hypergraphs; ground-truth, predicted, and unknown count of products in each basket. The hypergraph with unknown counts indicates a situation in which you only know if the product is in a basket but don't know if there is a duplicate purchase. As a result, the second best result after the case of the ground-truth in this product return prediction task also supports the usefulness of identifying edge-dependent node labels by our \method in real-life.
% We compare the competitors described detail in ~\cite{li2018tail}. Additionally, we experiment HyperGo on the uniform weighted hypergraph where the existence of multiple products within the same basket cannot be known.


% Previous ========================================================================================
% We train our model with free-for-all matches by splitting them into train/valid/test. Since the scores of players in each match are continuous value in range 0 to 1, we normalize the scores for each match and then the scores are binned into 5 bins containing 1/5 (20\%) of the total in the training set. Therefore, the binning index corresponds to the edge-dependent node labels. 
% After training our model, we predict all the scores of players in free-for-all matches by replacing binning index with the corresponding value. The final ranking of the total players are determined by the stationary distribution of the random walks on hypergraphs with the predicted edge-dependent vertex weights as proposed in ~\cite{chitra2019random}. In the evaluation on the 1-v-1 matches, we predict the winner as the one with the higher final ranking.

% \noindent\textbf{Data.} Since the datasets used in ~\cite{chitra2019random} have either trivial edge-dependent node labels such as tf-idf or do not have answer for clustering, we make a dataset extracted from Coauthorship-DBLP. We extract hyperedges which belong to only one category among computer science, data engineering, software engineering and theory, and choose one connected component. It consists of 33,050 hyperedges (publications) and 52,560 nodes (authors). The edge-dependent node labels indicate the position of authors in each publication and classified into three as described in Section~\ref{benchmark_dataset}, and hyperedges are classified into four categories.
% \textbf{Training.} We train our \method to predict the positions of authors in each publication. After predicting all positions of authors in publications, we weight the authors according to the positions by following~\cite{chitra2019random}. 
% \begin{equation*}
%     \gamma_{e}(v) = \begin{cases}
%  2 & \text{ if the vertex } v \text{ is the first or last author of publication} \\
%  1 & \text{ if the vertex } v \text{ is a middle author of publication}
% \end{cases}
% \end{equation*}
% Then we apply clustering algorithm (RDC-Spec)~\cite{hayashi2020hypergraph} on this hypergraphs. Specifically, the stationary distribution of random walks with consideration of edge-dependent node weights is used for spectral clustering.
% \textbf{Results.} We compare the performance of RDC-Spec on three different hypergraphs; ground-truth, predicted and unknown author positions while unifying how to weigh author positions as above. In that the result of using our \method comes between knowing the ground-truth and not knowing at all, we could assert that it is certainly beneficial to find out positions of authors in each hyperedge, i.e. edge-dependent node labels.


% Previous ========================================================================================
% To show the usefulness of our \method in real-world applications, we also evaluate our \method on a downstream task of ranking aggregation. The aim of the ranking aggregation task is to predict a complete ranking when only partial rankings are known. As an example of this task, we consider ranking players in a multiplayer game. Here, for every matches, the rankings of the participants are determined. If we exactly figure out the rakings of the entire players, we can make more exciting game by matching players into competitive matches.

% We experiment on real-world datasets of Halo 2 games in the same way described in ~\cite{chitra2019random}. The Halo 2 presented in the TrueSkill paper~\cite{herbrich2006trueskill} is composed of two kinds of matches. The free-for-all matches are where up to 8 players play together and are used for constructing rankings of all players, i.e. training dataset. The 1-v-1 matches are where only two players compete and are used for evaluating how correct the method predicts the winner well.
% In addition, we add competitors to support the importance of knowing the hyperedge-dependent node labels (otherwise we can also refer this as hyperedge-dependent node weights in this task). The \textit{uniform hypergraph} shows the result of replacing the hyperedge-dependent node weight matrix into the incidence matrix in the above process.
% The result of applying \method show better performance than MC3, random walks on the clique graph and hypergraph with uniform node weights. Its performance is quite comparable to TrueSkill and the result from original hypergraph with edge-dependent node weights. Similar to ~\cite{chitra2019random}, the ranking aggregation via applying our \method can also catch some missing information of TrueSkill.

% To apply our \method in this experiment, we train our \method to predict the score of players in each match. In detail, the scores are normalized in each match and then the normalized scores from the training dataset are binned into 5 bins each containing 1/5 (20\%) of the total. When the vertices are the players and the hyperedges are the free-for-all matches, the binning index can be corresponded to the edge-dependent node labels. Likewise, we train our \method by converting prediction of edge-dependent scores into that of edge-dependent labels. After training, we predict all the scores of players in free-for-all matches. Based on these scores, the final ranking of the total players are determined by the stationary distribution of the random walks on hypergraphs with edge-dependent vertex weights as proposed in ~\cite{chitra2019random}. In the evaluation on the 1-v-1 matches, we predict the winner as the one with the higher final ranking.

% In addition, we add competitors to support the importance of knowing the hyperedge-dependent node labels (otherwise we can also refer this as hyperedge-dependent node weights in this task). The \textit{uniform hypergraph} shows the result of replacing the hyperedge-dependent node weight matrix into the incidence matrix in the above process.

% The result of applying \method show better performance than MC3, random walks on the clique graph and hypergraph with uniform node weights. Its performance is quite comparable to TrueSkill and the result from original hypergraph with edge-dependent node weights. Similar to ~\cite{chitra2019random}, the ranking aggregation via applying our \method can also catch some missing information of TrueSkill.

% Previous Table ==================================================================================
% \begin{table}[t]
%     \vspace{-3mm}
% 	\begin{center}
% 		\caption{\label{tab:datasets}Summary of real-world hypergraphs.}
% 		%\vspace{-1mm}
% 		\scalebox{0.7}{
% 		    \begin{tabular}{l| c | c | c | c | c | c}
% 				\toprule
% 				%\textbf{Dataset} & \bigcell{c}{$|\SV|$} & \bigcell{c}{$|\SE|$} & \bigcell{c}{MAX.\\d($v$)} & \bigcell{c}{MAX.\\|$e$|} & \bigcell{c}{\# Classes} \\ 
% 				\multirow{2}{*}{Statistics} & \multicolumn{2}{c}{Co-Authorship} &  \multicolumn{2}{c}{Email} & \multicolumn{2}{c}{StackOverflow} \\ 
% 				 & DBLP & AMinerAuthor & Enron & Eu & Biology & Physics \\ 
% 				\midrule
% 				\# Nodes & 108,484 & 1,712,433 & 21,251 & 986 & 15,490 & 80,936 \\
% 				\# Hyperedges & 91,266 & 2,037,605 & 101,124 & 209,508 & 26,823 & 200,811 \\
% 				MAX. Node degree & 236 & 752 & 18,168 & 8,659 & 1,318 & 6,332 \\
% 				MAX. Hyperedge size & 36 & 115 & 948 & 59 & 12 & 48 \\
% 				\# Node classes & 3 & 3 & 3 & 2 & 3 & 3 \\
% 				\bottomrule
% 			\end{tabular}}
% 	\end{center}
% 	%\vspace{-4mm}
% \end{table}

% \begin{table*}[h]
%     \begin{center}
%         \caption{\label{tab:expresult} F1 Micro and Macro Score}
%         \scalebox{0.6}{
%             \begin{tabular}{l|c cc c cc c cc c cc c cc c cc}
%             \toprule
%             \multirow{2}{*}{Models} && \multicolumn{2}{c}{Coauthorship-DBLP} && \multicolumn{2}{c}{Coauthorship-AMiner} && \multicolumn{2}{c}{Email-Enron} && \multicolumn{2}{c}{Email-Eu} && \multicolumn{2}{c}{StackOverflow-Biology} && \multicolumn{2}{c}{StackOverflow-Physics} \\
%             \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13} \cmidrule{15-16} \cmidrule{18-19}\\
%             && Micro-F1 & Macro-F1 && Micro-F1 & Macro-F1 && Micro-F1 & Macro-F1 && Micro-F1 & Macro-F1 && Micro-F1 & Macro-F1 && Micro-F1 & Macro-F1 \\
%             \midrule
%             Baseline0 && 0.333 $$\pm$$ 0.001 & 0.330 $\pm$ 0.001 && 0.334 $\pm$ 0.000 & 0.332 $\pm$ 0.000 && 0.334 $\pm$ 0.001 & 0.300 $\pm$ 0.001 && 0.500 $\pm$ 0.001 & 0.493 $\pm$ 0.001 && 0.335 $\pm$ 0.000 & 0.326 $\pm$ 0.000 && 0.333 $\pm$ 0.001 & 0.322 $\pm$ 0.001 \\
%             Baseline1 && 0.346 $\pm$ 0.001 & 0.332 $\pm$ 0.001 && 0.339 $\pm$ 0.000 & 0.333 $\pm$ 0.000 && 0.439 $\pm$ 0.001 & 0.333 $\pm$ 0.001 && 0.525 $\pm$ 0.001 & 0.499 $\pm$ 0.001 && 0.368 $\pm$ 0.001 & 0.334 $\pm$ 0.003 && 0.370 $\pm$ 0.000 & 0.332 $\pm$ 0.000 \\
%             \midrule
%             HNHN && 0.486 $\pm$ 0.002 & 0.476 $\pm$ 0.003 && 0.521 $\pm$ 0.002 & 0.515 $\pm$ 0.002 && 0.726 $\pm$ 0.040 & 0.620 $\pm$ 0.041 && 0.642 $\pm$ 0.004 & 0.548 $\pm$ 0.015 && 0.636 $\pm$ 0.006 & 0.585 $\pm$ 0.001 && 0.446 $\pm$ 0.001 & 0.372 $\pm$ 0.003 \\ 
%             HGNN && 0.542 $\pm$ 0.001 & 0.519 $\pm$ 0.003 && 0.566 $\pm$ 0.003 & 0.553 $\pm$ 0.001 && 0.723 $\pm$ 0.005 & 0.673 $\pm$ 0.003 && 0.633 $\pm$ 0.001 & 0.530 $\pm$ 0.008 && 0.690 $\pm$ 0.001 & 0.626 $\pm$ 0.006 && 0.688 $\pm$ 0.005 & 0.631 $\pm$ 0.003 \\ 
%             HCHA && 0.454 $\pm$ 0.007 & 0.360 $\pm$ 0.045 && - & - && 0.668 $\pm$ 0.005 & 0.465 $\pm$ 0.001 && 0.621 $\pm$ 0.000 & 0.497 $\pm$ 0.001 && 0.587 $\pm$ 0.002 & 0.417 $\pm$ 0.003 && 0.622 $\pm$ 0.004 & 0.481 $\pm$ 0.008 \\ 
%             HAT && 0.505 $\pm$ 0.002 & 0.486 $\pm$ 0.006 && 0.541 $\pm$ 0.001 & 0.531 $\pm$ 0.003 && 0.817 $\pm$ 0.001 & 0.755 $\pm$ 0.003 && 0.669 $\pm$ 0.001 & 0.640 $\pm$ 0.003 && 0.662 $\pm$ 0.005 & 0.609 $\pm$ 0.005 && 0.709 $\pm$ 0.004 & 0.642 $\pm$ 0.009 \\ 
%             UniGCNII && 0.497 $\pm$ 0.004 & 0.476 $\pm$ 0.003 && 0.521 $\pm$ 0.000 & 0.507 $\pm$ 0.001 && 0.741 $\pm$ 0.003 & 0.658 $\pm$ 0.012 && 0.633 $\pm$ 0.002 & 0.560 $\pm$ 0.012 && 0.605 $\pm$ 0.004 & 0.425 $\pm$ 0.004 && 0.664 $\pm$ 0.026 & 0.487 $\pm$ 0.019 \\ 
%             \midrule
%             SetTransformer && 0.474 $\pm$ 0.063 & 0.324 $\pm$ 0.158 && 0.595 $\pm$ 0.008 & 0.584 $\pm$ 0.004 && 0.684 $\pm$ 0.013 & 0.536 $\pm$ 0.041 && 0.671 $\pm$ 0.001 & 0.639 $\pm$ 0.001 && 0.698 $\pm$ 0.003 & 0.638 $\pm$ 0.001 && 0.756 $\pm$ 0.013 & 0.660 $\pm$ 0.013 \\
%             AllSetTransformer && 0.526 $\pm$ 0.003 & 0.520 $\pm$ 0.003 && 0.581 $\pm$ 0.000 & 0.572 $\pm$ 0.001 && 0.807 $\pm$ 0.001 & 0.735 $\pm$ 0.001 && 0.669 $\pm$ 0.001 & 0.639 $\pm$ 0.001 && 0.718 $\pm$ 0.002 & 0.645 $\pm$ 0.003 && 0.759 $\pm$ 0.003 & 0.680 $\pm$ 0.006 \\ 
%             \midrule
%             \method w/o \WithinAttention && 0.583 $\pm$ 0.004 & 0.579 $\pm$ 0.003 && 0.612 $\pm$ 0.001 & 0.602 $\pm$ 0.001 && 0.819 $\pm$ 0.002 & 0.758 $\pm$ 0.006 && 0.665 $\pm$ 0.003 & 0.641 $\pm$ 0.005 && 0.727 $\pm$ 0.000 & 0.647 $\pm$ 0.010 && 0.756 $\pm$ 0.001 & 0.671 $\pm$ 0.012 \\ 
%             \method w/o \PE && 0.589 $\pm$ 0.003 & 0.582 $\pm$ 0.003 && \textbf{0.629} $\pm$ 0.002 & \textbf{0.622} $\pm$ 0.002 && 0.825 $\pm$ 0.000 & \textbf{0.762} $\pm$ 0.004 && 0.670 $\pm$ 0.000 & 0.638 $\pm$ 0.003 && 0.734 $\pm$ 0.004 & \textbf{0.680} $\pm$ 0.002 && 0.765 $\pm$ 0.002 & 0.689 $\pm$ 0.008 \\ 
%             \midrule
%             \midrule
%             \method && \textbf{0.606} $\pm$ 0.002 & \textbf{0.596} $\pm$ 0.001 && 0.627 $\pm$ 0.004 & 0.621 $\pm$ 0.006 && \textbf{0.826} $\pm$ 0.001 & 0.760 $\pm$ 0.003 && \textbf{0.672} $\pm$ 0.000 & \textbf{0.640} $\pm$ 0.004 && \textbf{0.738} $\pm$ 0.001 & \textbf{0.680} $\pm$ 0.003 && \textbf{0.773} $\pm$ 0.002 & \textbf{0.707} $\pm$ 0.002 \\
%             \bottomrule
%         \end{tabular}}
%     \end{center}
% \end{table*}

% \begin{table*}[h]
%     \begin{center}
%         \caption{\label{tab:jsdresult} JS-Divergence}
%         \scalebox{0.72}{
%             \begin{tabular}{c |c c c c c c c|c c c c||c c}
%             \toprule
%             DataSet && HNHN & HGNN & HCHA & HAT & UniGCNII & HST & AST &&& \method\\
%             \midrule
%             Coauth-DBLP &&  0.451 $\pm$ 0.381 &  0.391 $\pm$ 0.381 &  0.451 $\pm$ 0.381 &  0.427 $\pm$ 0.382 &  0.450 $\pm$ 0.382 &&&  0.444 $\pm$ 0.381 &  0.423 $\pm$ 0.383 &&&  \textbf{0.233} $\pm$ 0.253\\ 
%             Coauth-AMiner &&  0.438 $\pm$ 0.385 &  0.372 $\pm$ 0.382 & - &  0.413 $\pm$ 0.386 &  0.423 $\pm$ 0.385 &&&  0.357 $\pm$ 0.381 &  0.375 $\pm$ 0.384 &&&  \textbf{0.330} $\pm$ 0.377\\ 
%             Email-Enron &&  0.159 $\pm$ 0.259 &  0.214 $\pm$ 0.277 &  0.290 $\pm$ 0.317 &  0.156 $\pm$ 0.258 &  0.188 $\pm$ 0.268 &&&  0.272 $\pm$ 0.314 &  0.162 $\pm$ 0.262 &&&  \textbf{0.136} $\pm$ 0.241\\ 
%             Email-Eu &&  0.234 $\pm$ 0.175 &  0.291 $\pm$ 0.179 &  0.268 $\pm$ 0.183 &  \textbf{0.152} $\pm$ 0.158 &  0.297 $\pm$ 0.181 &&&  0.160 $\pm$ 0.158 &  0.157 $\pm$ 0.156 &&&  0.155 $\pm$ 0.155\\ 
%             Stack-Biology &&  0.273 $\pm$ 0.364 &  0.202 $\pm$ 0.325 &  0.221 $\pm$ 0.334 &  0.237 $\pm$ 0.348 &  0.261 $\pm$ 0.362 &&&  0.197 $\pm$ 0.325 &  0.186 $\pm$ 0.317 &&&  \textbf{0.155} $\pm$ 0.293\\ 
%             Stack-Physics &&  0.303 $\pm$ 0.366 &  0.215 $\pm$ 0.324 &  0.288 $\pm$ 0.359 &  0.230 $\pm$ 0.337 &  0.298 $\pm$ 0.360 &&&  0.160 $\pm$ 0.289 &  0.168 $\pm$ 0.299 &&&  \textbf{0.140} $\pm$ 0.275\\ 
%             \bottomrule
%         \end{tabular}}
%     \end{center}
% \end{table*}
% \begin{table*}[h]
%     \begin{center}
%         \caption{\label{tab:jsdresult} JS-Divergence}
%         \scalebox{0.65}{
%             \begin{tabular}{l|c c c c c c}
%             \toprule
%             Models & Coauthorship-DBLP & Coauthorship-AMiner & Email-Enron & Email-Eu & StackOverflow-Biology & StackOverflow-Physics \\
%             \midrule
%             HNHN & 0.451 $\pm$ 0.381 & 0.438 $\pm$ 0.385 & 0.159 $\pm$ 0.259 & 0.234 $\pm$ 0.175 & 0.273 $\pm$ 0.364 & 0.303 $\pm$ 0.366 \\ 
%             HGNN & 0.391 $\pm$ 0.381 & 0.372 $\pm$ 0.382 & 0.214 $\pm$ 0.277 & 0.291 $\pm$ 0.179 & 0.202 $\pm$ 0.325 & 0.215 $\pm$ 0.324 \\ 
%             HCHA & 0.451 $\pm$ 0.381 & - &  0.290 $\pm$ 0.317 & 0.268 $\pm$ 0.183 & 0.221 $\pm$ 0.334 & 0.288 $\pm$ 0.359 \\ 
%             HAT & 0.427 $\pm$ 0.382 & 0.413 $\pm$ 0.386 & 0.156 $\pm$ 0.258 & 0.152 $\pm$ 0.158 & 0.157 $\pm$ 0.232 & 0.230 $\pm$ 0.337 \\ 
%             UniGCNII & 0.450 $\pm$ 0.382 & 0.423 $\pm$ 0.385 & 0.188 $\pm$ 0.268 & 0.297 $\pm$ 0.181 & 0.261 $\pm$ 0.362 & 0.298 $\pm$ 0.360 \\ \midrule
%             SetTransformer & 0.444 $\pm$ 0.381 & 0.357 $\pm$ 0.381 & 0.272 $\pm$ 0.314 & 0.160 $\pm$ 0.158 & 0.197 $\pm$ 0.325 & 0.160 $\pm$ 0.289 \\ 
%             AllSetTransformer & 0.423 $\pm$ 0.383 & 0.375 $\pm$ 0.384 & 0.162 $\pm$ 0.262 & 0.157 $\pm$ 0.156 & 0.186 $\pm$ 0.317 & 0.168 $\pm$ 0.299 \\ 
%             \midrule
%             \method w/o \WithinAttention & 0.373 $\pm$ 0.383 & 0.349 $\pm$ 0.381 & 0.148 $\pm$ 0.249 &\textbf{ 0.140} $\pm$ 0.151 & 0.160 $\pm$ 0.297 & 0.155 $\pm$ 0.287 \\ 
%             \method w/o \PE & 0.369 $\pm$ 0.382 & 0.330 $\pm$ 0.377 & 0.143 $\pm$ 0.246 & 0.156 $\pm$ 0.157 & 0.157 $\pm$ 0.295 & 0.151 $\pm$ 0.284 \\ 
%             \midrule
%             \midrule
%             \method & \textbf{0.352} $\pm$ 0.380 & \textbf{0.327} $\pm$ 0.377 & \textbf{0.136} $\pm$ 0.240 & 0.141 $\pm$ 0.154 & \textbf{0.154} $\pm$ 0.292 & \textbf{0.143} $\pm$ 0.278 \\ 
%             \bottomrule
%         \end{tabular}}
%     \end{center}
% \end{table*}

% \begin{table*}[h]
%     \begin{center}
%         \caption{\label{tab:jsdavg}}
%         \scalebox{0.65}{
%             \begin{tabular}{l|c c c c c | c c c c || c}
%             \toprule
%              & HNHN & HGNN & HCHA & HAT & UniGCNII & SetTransformer & AllSetTransformer & \method w/o \WithinAttention & \method w/o \PE & \method \\
%             \midrule
%             Diff. in Label Dist. & 0.183 & 0.201 & 0.454 & 0.108 & 0.281 & 0.264 & 0.105 & 0.095 & \textbf{0.078} & 0.093\\
%             JS Divergence & 0.310 & 0.281 & 0.303 & 0.256 & 0.319 & 0.265 & 0.245 & 0.221 & 0.218 & \textbf{0.209}\\
%             \bottomrule
%         \end{tabular}}
%     \end{center}
% \end{table*}

% \begin{table*}[h]
%     \begin{center}
%         \caption{\label{tab:ablresult} Ablation Study}
%         \scalebox{0.65}{
%             \begin{tabular}{l|c cc c cc c|l|c cc c cc}
%             \toprule
%             \multirow{2}{*}{Models} && \multicolumn{2}{c}{Coauthorship-DBLP} && \multicolumn{2}{c}{StackOverflow-Biology} && \multirow{2}{*}{Models}  && \multicolumn{2}{c}{Coauthorship-DBLP} && \multicolumn{2}{c}{StackOverflow-Biology}\\
%             %\cmidrule{3-4} \cmidrule{6-7} \cmidrule{11-12} \cmidrule{14-15} \\
%             && Micro-F1 & Macro-F1 && Micro-F1 & Macro-F1 && && Micro-F1 & Macro-F1 && Micro-F1 & Macro-F1\\
%             \midrule
%             HNHN && 0.486 $\pm$ 0.002 & 0.476 $\pm$ 0.003 && 0.636 $\pm$ 0.006 & 0.585 $\pm$ 0.001 && \method w/ PMA && 0.591 $\pm$ 0.002 & 0.574 $\pm$ 0.004 && 0.734 $\pm$ 0.002 & 0.684 $\pm$ 0.004 \\ 
%             \method + HNHN && 0.529 $\pm$ 0.003 & 0.509 $\pm$ 0.004 && 0.696 $\pm$ 0.004 & 0.635 $\pm$ 0.008 && \method w/ AvgAgg && 0.591 $\pm$ 0.000 & 0.570 $\pm$ 0.001 && \textbf{0.743} $\pm$ 0.002 & \textbf{0.689} $\pm$ 0.005 \\ 
%             \midrule
%             \midrule
%             \method && \textbf{0.602} $\pm$ 0.001 & \textbf{0.590} $\pm$ 0.004 && \textbf{0.738} $\pm$ 0.000 & \textbf{0.674} $\pm$ 0.004 && \method && \textbf{0.602} $\pm$ 0.001 & \textbf{0.590} $\pm$ 0.004 && 0.738 $\pm$ 0.000 & 0.674 $\pm$ 0.004 \\ 
%             \bottomrule
%         \end{tabular}}
%     \end{center}
% \end{table*}

% 10.05 ---------------------------------------------------------------------------------------------------------------------
% \begin{table*}[h]
%     \begin{center}
%         \caption{\label{tab:expresult} F1 Micro and Macro Score}
%         \scalebox{0.716}{
%             \begin{tabular}{c c |c c c c|c c c c c c c|c c c c||c c}
%             \toprule
%             \multicolumn{2}{c|}{DataSet} && BaselineU & BaselineP &&& HNHN & HGNN & HCHA & HAT & UniGCNII &&& HST & AST &&& \method\\ 
%             \midrule
%             \multirow{2}{*}{\shortstack{Coauth\\DBLP}} & MicroF1 && 0.333 $\pm$ 0.001 & 0.346 $\pm$ 0.001 &&& 0.486 $\pm$ 0.002 & 0.542 $\pm$ 0.001 & 0.454 $\pm$ 0.007 & 0.505 $\pm$ 0.002 & 0.497 $\pm$ 0.004 &&& 0.474 $\pm$ 0.063 & 0.526 $\pm$ 0.003 &&& \textbf{0.605} $\pm$ 0.002 \\
%             & MacroF1 && 0.330 $\pm$ 0.001 & 0.332 $\pm$ 0.001 &&& 0.476 $\pm$ 0.003 & 0.519 $\pm$ 0.003 & 0.360 $\pm$ 0.045 & 0.486 $\pm$ 0.006 & 0.476 $\pm$ 0.003 &&& 0.324 $\pm$ 0.158 & 0.520 $\pm$ 0.003 &&& \textbf{0.594} $\pm$ 0.003\\
%             \midrule
%             \multirow{2}{*}{\shortstack{Coauth\\AMiner}} & MicroF1 && 0.334 $\pm$ 0.000 & 0.339 $\pm$ 0.000 &&& 0.521 $\pm$ 0.002 & 0.566 $\pm$ 0.003 & - & 0.541 $\pm$ 0.001 & 0.521 $\pm$ 0.000 &&& 0.595 $\pm$ 0.008 & 0.581 $\pm$ 0.000 &&& \textbf{0.627} $\pm$ 0.004\\
%             & MacroF1 && 0.332 $\pm$ 0.000 & 0.333 $\pm$ 0.000 &&& 0.515 $\pm$ 0.002 & 0.553 $\pm$ 0.001 & - & 0.531 $\pm$ 0.003 & 0.507 $\pm$ 0.001 &&& 0.584 $\pm$ 0.004 & 0.572 $\pm$ 0.001 &&& \textbf{0.621} $\pm$ 0.006\\
%             \midrule
%             \multirow{2}{*}{\shortstack{Email\\Enron}} & MicroF1 && 0.334 $\pm$ 0.001 & 0.439 $\pm$ 0.001 &&& 0.726 $\pm$ 0.040 & 0.723 $\pm$ 0.005 & 0.668 $\pm$ 0.005 & 0.817 $\pm$ 0.001 & 0.741 $\pm$ 0.003 &&& 0.684 $\pm$ 0.013 & 0.807 $\pm$ 0.001 &&& \textbf{0.826} $\pm$ 0.001\\
%             & MacroF1 && 0.300 $\pm$ 0.001 & 0.333 $\pm$ 0.001 &&& 0.620 $\pm$ 0.041 & 0.673 $\pm$ 0.003 & 0.465 $\pm$ 0.001 & 0.755 $\pm$ 0.003 & 0.658 $\pm$ 0.012 &&& 0.536 $\pm$ 0.041 & 0.735 $\pm$ 0.001 &&& \textbf{0.760} $\pm$ 0.003\\
%             \midrule
%             \multirow{2}{*}{\shortstack{Email\\Eu}} & MicroF1 && 0.500 $\pm$ 0.001 & 0.525 $\pm$ 0.001 &&& 0.642 $\pm$ 0.004 & 0.633 $\pm$ 0.001 & 0.621 $\pm$ 0.000 & 0.669 $\pm$ 0.001 & 0.633 $\pm$ 0.002 &&& 0.671 $\pm$ 0.001 & 0.669 $\pm$ 0.001 &&& \textbf{0.672} $\pm$ 0.000\\
%             & MacroF1 && 0.493 $\pm$ 0.001 & 0.499 $\pm$ 0.001 &&& 0.548 $\pm$ 0.015 & 0.530 $\pm$ 0.008 & 0.497 $\pm$ 0.001 & 0.640 $\pm$ 0.003 & 0.560 $\pm$ 0.012 &&& 0.639 $\pm$ 0.001 & 0.639 $\pm$ 0.001 &&& \textbf{0.640} $\pm$ 0.004\\
%             \midrule
%             \multirow{2}{*}{\shortstack{Stack \\Biology}} & MicroF1 && 0.335 $\pm$ 0.000 & 0.368 $\pm$ 0.001 &&& 0.636 $\pm$ 0.006 & 0.690 $\pm$ 0.001 & 0.587 $\pm$ 0.002 & 0.659 $\pm$ 0.006 & 0.605 $\pm$ 0.004 &&& 0.698 $\pm$ 0.003 & 0.718 $\pm$ 0.002 &&& \textbf{0.738} $\pm$ 0.001\\
%             & MacroF1 && 0.326 $\pm$ 0.000 & 0.334 $\pm$ 0.003 &&& 0.585 $\pm$ 0.001 & 0.626 $\pm$ 0.006 & 0.417 $\pm$ 0.003 & 0.604 $\pm$ 0.008 & 0.425 $\pm$ 0.004 &&& 0.638 $\pm$ 0.001 & 0.645 $\pm$ 0.003 &&& \textbf{0.680} $\pm$ 0.003\\
%             \midrule
%             \multirow{2}{*}{\shortstack{Stack \\Physics  }} & MicroF1 && 0.333 $\pm$ 0.001 & 0.370 $\pm$ 0.000 &&& 0.446 $\pm$ 0.001 & 0.688 $\pm$ 0.005 & 0.622 $\pm$ 0.004 & 0.709 $\pm$ 0.004 & 0.664 $\pm$ 0.026 &&& 0.756 $\pm$ 0.013 & 0.759 $\pm$ 0.003 &&& \textbf{0.773} $\pm$ 0.002\\
%             & MacroF1 && 0.322 $\pm$ 0.001 & 0.332 $\pm$ 0.000 &&& 0.372 $\pm$ 0.003 & 0.631 $\pm$ 0.003 & 0.481 $\pm$ 0.008 & 0.642 $\pm$ 0.009 & 0.487 $\pm$ 0.019 &&& 0.660 $\pm$ 0.013 & 0.680 $\pm$ 0.006 &&& \textbf{0.707} $\pm$ 0.002\\
%             \bottomrule
%         \end{tabular}}
%     \end{center}
% \end{table*}
% \begin{table*}[h]
%     \begin{center}
%         \caption{\label{tab:jsdresult} JS-Divergence}
%         \scalebox{0.72}{
%             \begin{tabular}{c c|c c c c|c c c c c c c|c c c c||c c}
%             \toprule
%             \multicolumn{2}{c|}{DataSet} && BaselineU & BaselineP &&& HNHN & HGNN & HCHA & HAT & UniGCNII &&& HST & AST &&& \method\\
%             \midrule
%             Coauth & DBLP && 0.532 $\pm$ 0.360 &  0.518 $\pm$ 0.364 &&& 0.451 $\pm$ 0.381 &  0.391 $\pm$ 0.381 &  0.451 $\pm$ 0.381 &  0.427 $\pm$ 0.382 &  0.450 $\pm$ 0.382 &&&  0.444 $\pm$ 0.381 &  0.423 $\pm$ 0.383 &&&  \textbf{0.233} $\pm$ 0.253\\ 
%             Coauth & AMiner && 0.529 $\pm$ 0.363 &  0.523 $\pm$ 0.364 &&& 0.438 $\pm$ 0.385 &  0.372 $\pm$ 0.382 & - &  0.413 $\pm$ 0.386 &  0.423 $\pm$ 0.385 &&&  0.357 $\pm$ 0.381 &  0.375 $\pm$ 0.384 &&&  \textbf{0.330} $\pm$ 0.377\\ 
%             Email & Enron && 0.486 $\pm$ 0.270 &  0.395 $\pm$ 0.284 &&&  0.159 $\pm$ 0.259 &  0.214 $\pm$ 0.277 &  0.290 $\pm$ 0.317 &  0.156 $\pm$ 0.258 &  0.188 $\pm$ 0.268 &&&  0.272 $\pm$ 0.314 &  0.162 $\pm$ 0.262 &&&  \textbf{0.136} $\pm$ 0.241\\ 
%             Email & Eu && 0.199 $\pm$ 0.202 &  0.164 $\pm$ 0.193 &&& 0.234 $\pm$ 0.175 &  0.291 $\pm$ 0.179 &  0.268 $\pm$ 0.183 &  \textbf{0.152} $\pm$ 0.158 &  0.297 $\pm$ 0.181 &&&  0.160 $\pm$ 0.158 &  0.157 $\pm$ 0.156 &&&  0.155 $\pm$ 0.155\\ 
%             Stack & Biology && 0.536 $\pm$ 0.361 &  0.467 $\pm$ 0.375 &&& 0.273 $\pm$ 0.364 &  0.202 $\pm$ 0.325 &  0.221 $\pm$ 0.334 &  0.237 $\pm$ 0.348 &  0.261 $\pm$ 0.362 &&&  0.197 $\pm$ 0.325 &  0.186 $\pm$ 0.317 &&&  \textbf{0.155} $\pm$ 0.293\\ 
%             Stack & Physics && 0.532 $\pm$ 0.350 &  0.482 $\pm$ 0.361 &&& 0.303 $\pm$ 0.366 &  0.215 $\pm$ 0.324 &  0.288 $\pm$ 0.359 &  0.230 $\pm$ 0.337 &  0.298 $\pm$ 0.360 &&&  0.160 $\pm$ 0.289 &  0.168 $\pm$ 0.299 &&&  \textbf{0.140} $\pm$ 0.275\\ 
%             \bottomrule
%         \end{tabular}}
%     \end{center}
% \end{table*}

% \begin{table*}[h]
%     \begin{center}
%         \caption{\label{tab:ablresult} Ablation Study}
%         \scalebox{0.72}{
%             \begin{tabular}{c c|c c c c c|| c c|c c c c}
%             \toprule
%             \multicolumn{2}{c|}{DataSet} && w/o \WithinAttention & w/o \PE & \method && \multicolumn{2}{c|}{DataSet} && w/o \WithinAttention & w/o \PE & \method \\
%             %\cmidrule{3-4} \cmidrule{6-7} \cmidrule{11-12} \cmidrule{14-15} \\
%             \midrule
%             \multirow{2}{*}{\shortstack{Coauth\\DBLP}} & MicroF1 && 0.583 $\pm$ 0.004 & 0.589 $\pm$ 0.003 & \textbf{0.605} $\pm$ 0.002 &&
%             \multirow{2}{*}{\shortstack{Email\\Eu}} & MicroF1 && 0.665 $\pm$ 0.003 & 0.670 $\pm$ 0.000 & \textbf{0.672} $\pm$ 0.000 \\
%              & MacroF1 && 0.579 $\pm$ 0.003 & 0.582 $\pm$ 0.003 & \textbf{0.594} $\pm$ 0.003 &&
%              & MacroF1 && \textbf{0.641} $\pm$ 0.005 & 0.638 $\pm$ 0.003 & 0.640 $\pm$ 0.004 \\
%             \midrule
%             \multirow{2}{*}{\shortstack{Coauth\\AMiner}} & MicroF1 && 0.612 $\pm$ 0.001 & \textbf{0.629} $\pm$ 0.002 & 0.627 $\pm$ 0.004 &&
%             \multirow{2}{*}{\shortstack{Stack\\Biology}} & MicroF1 && 0.727 $\pm$ 0.000 & 0.734 $\pm$ 0.004 & \textbf{0.738} $\pm$ 0.001 \\
%              & MacroF1 && 0.602 $\pm$ 0.001 & \textbf{0.622} $\pm$ 0.002 & 0.621 $\pm$ 0.006 &&
%              & MacroF1 && 0.647 $\pm$ 0.010 & \textbf{0.680} $\pm$ 0.002 & \textbf{0.680} $\pm$ 0.003 \\
%             \midrule
%             \multirow{2}{*}{\shortstack{Email\\Enron}} & MicroF1 && 0.819 $\pm$ 0.002 & 0.825 $\pm$ 0.000 & \textbf{0.826} $\pm$ 0.001 &&
%             \multirow{2}{*}{\shortstack{Stack\\Biology}} & MicroF1 && 0.756 $\pm$ 0.001 & 0.765 $\pm$ 0.002 & \textbf{0.773} $\pm$ 0.002 \\
%              & MacroF1 && 0.758 $\pm$ 0.006 & \textbf{0.762} $\pm$ 0.004 & 0.760 $\pm$ 0.003 &&
%              & MacroF1 && 0.671 $\pm$ 0.012 & 0.689 $\pm$ 0.008 & \textbf{0.707} $\pm$ 0.002 \\
%             \bottomrule
%         \end{tabular}}
%     \end{center}
% \end{table*}
% 10.05------------------------------------------------------------------------------------------------------------------
% \begin{table}[t]
% 	\caption{\label{tab:ranking} Ranking Aggregation}
% 	\scalebox{0.88}{
% 		\begin{tabular}{l|c}
% 			\toprule
% 			Method & Accuracy \\
% 			\midrule
% 			TrueSkill & \textbf{73.4} \% \\
% 			Hypergraph & 71.1 \% \\
% 			\textbf{Hypergraph w/ \method} & \underline{71.8} \% \\
% 			Clique Graph & 61.1 \% \\
% 			Uniform Weighted Hypergraph & 53.2 \% \\
% 			MC3 & 52.9 \% \\
% 			\bottomrule
% 		\end{tabular}}
% \end{table}
% \begin{table}[t]
% 	\caption{\label{tab:clustering} Clustering NMI Score}
% 	\scalebox{0.85}{
% 		\begin{tabular}{l|c}
% 			\toprule
% 			Method & NMI Score\\
% 			\midrule
% 			Hypergraph & \textbf{0.2209} \\
% 			\textbf{Hypergraph w/ \method} & \underline{0.2146} \\
% 			Uniform Weighted Hypergraph & 0.1634 \\
% 			\bottomrule
% 		\end{tabular}}
% \end{table}
% \begin{table}[t]
% 	\caption{\label{tab:returnpredict} Return Prediction}
% 	\scalebox{0.85}{
% 		\begin{tabular}{l|c}
% 			\toprule
% 			Method & Precision\\
% 			\midrule
% 			HyperGO & \textbf{0.7553}\\
% 			\textbf{HyperGO w/ \method} & \underline{0.7536} \\
% 			Uniform Weighted Hypergraph &  0.7526 \\ 
% 			\bottomrule
% 		\end{tabular}}
% \end{table}

==> backup/080conclusion.tex <==
In this work, we propose the edge-dependent node label classification problem, which is a new benchmark task for hypergraph neural networks with various real-life applications. In order to tackle this problem, we devise \method, a hypergraph neural network for considering edge-dependent relationships between pairs of nodes within each hyperedge.
In our experiments with $6$ real-world hypergraphs,  \method consistently outperformed 9 competitors.
% Future research directions include could consider reducing the complexity of \method further or analyzing the effectiveness of \method in other problems. 
Our contributions are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item \textbf{New Problem}: We formulate the edge-dependent node label classification problem with six real-world benchmark datasets and three concrete applications. 
    \item \textbf{Effective Model}: We propose \method, a novel hypergraph neural network equipped with the \WithinAttention module and \PE. They are designed to capture edge-dependent relationships between pairs of nodes within each hyperedge.
    \item \textbf{Extensive Experiment}: We compared \method with $9$ competitors in our benchmark datasets. We also showed that every component of \method is effective through extensive ablation studies.
    In addition, we demonstrated the usefulness of \method in three applications.%
    
\end{itemize}
For reproducibility, the code and data are available at \cite{github}.

==> backup/dfn.tex <==
\newcommand\red[1]{\textcolor{red}{#1}}
\newcommand\blue[1]{\textcolor{blue}{#1}}
\newcommand\gray[1]{\textcolor{gray}{#1}}
\newcommand\kijung[1]{\textcolor{red}{[Kijung: #1]}}
\newcommand\minyoung[1]{\textcolor{blue}{#1}}
\newcommand\geon[1]{\textcolor{brown}{#1}}

\newcommand{\smallsection}[1]{{\vspace{0.02in} \noindent {{\underline{\smash{\bf #1.}}}}}}
\newtheorem{obs}{\textbf{Observation}}
\newtheorem{defn}{\textbf{Definition}}
\newtheorem{thm}{\textbf{Theorem}}
\newtheorem{axm}{\textbf{Axiom}}
\newtheorem{lma}{\textbf{Lemma}}
\newtheorem{cor}{\textbf{Corollary}}
\newtheorem{problem}{\textbf{Problem}}
\newtheorem{pro}{\textbf{Problem}}
% \newtheorem{proof}{\textbf{proof}}

\newcommand\und[1]{\underline{#1}}

\newcommand{\SM}{\mathcal{M}}%
\newcommand{\SG}{\mathcal{G}}%
\newcommand{\SSS}{\mathcal{S}}%
\newcommand{\SV}{\mathcal{V}}%
\newcommand{\SE}{\mathcal{E}}%
\newcommand{\SL}{\mathcal{L}}%
\newcommand{\SGH}{\mathcal{\hat{G}}}%
\newcommand{\SEH}{\mathcal{\hat{E}}}%
\newcommand{\SVH}{\mathcal{\hat{V}}}%
\newcommand{\SEVH}{\SE({\SVH})}%
\newcommand{\SVEH}{\SV({\SEH})}%
%\newcommand{\SES}{\SE_{\SSS}}%
%\newcommand{\SGS}{\SG_{\SSS}}%
\newcommand{\SD}{\mathcal{D}}%

\newcommand{\fhat}{\hat{f}}%
\newcommand{\flargehat}{\hat{F}}%
\newcommand{\yhat}{\hat{y}}%

\newcommand{\Ghat}{\SGH=(\SVH,\SEH)}%
\newcommand{\Glong}{\SG=(\SV,\SE)}%
%\newcommand{\GS}{\SGS=(\SSS,\SES)}%

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


\newcommand{\method}{\textsc{WHATsNet}\xspace}
\newcommand{\attention}{\textsc{ATT}\xspace}
\newcommand{\aggregation}{\textsc{AGG}\xspace}
\newcommand{\MultiheadAtt}{\textsc{MAB}\xspace}
\newcommand{\WithinAttentionFull}{within attention\xspace}
\newcommand{\WithinAttention}{\textsc{WithinATT}\xspace}
\newcommand{\PE}{\textsc{WithinOrderPE}\xspace}
% \newcommand{\PE}{\textsc{PE}\xspace}

\newcommand{\methodgrid}{\textsc{MiDaS-Grid}\xspace}
\newcommand{\methodauto}{\textsc{MiDaS}\xspace}

\definecolor{myred}{RGB}{195, 79, 82}
\definecolor{mygreen}{RGB}{86, 167 104}
\definecolor{myblue}{RGB}{74, 113 175}

\newcommand{\bigcell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

% Algorithm
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
